ScImage: How Good Are Multimodal Large Language Models at Scientific Text-to-Image Generation?

Multimodal large language models (LLMs) have demonstrated impressive capabilities in generating high-quality images from textual instructions. However, their performance in generating scientific images--a critical application for accelerating scientific progress--remains underexplored. In this work, we address this gap by introducing ScImage, a benchmark designed to evaluate the multimodal capabilities of LLMs in generating scientific images from textual descriptions. ScImage assesses three key dimensions of understanding: spatial, numeric, and attribute comprehension, as well as their combinations, focusing on the relationships between scientific objects (e.g., squares, circles). We evaluate five models, GPT-4o, Llama, AutomaTikZ, Dall-E, and StableDiffusion, using two modes of output generation: code-based outputs (Python, TikZ) and direct raster image generation. Additionally, we examine four different input languages: English, German, Farsi, and Chinese. Our evaluation, conducted with 11 scientists across three criteria (correctness, relevance, and scientific accuracy), reveals that while GPT-4o produces outputs of decent quality for simpler prompts involving individual dimensions such as spatial, numeric, or attribute understanding in isolation, all models face challenges in this task, especially for more complex prompts.

==> latex/other_commands_orig.tex <==
%\usepackage{xcolor}
\usepackage{fontawesome}
\usepackage{hyperref}
\usepackage{url}
\usepackage{times}
\usepackage{latexsym}
\usepackage{lscape}
\usepackage[dvipsnames]{xcolor}
\usepackage[export]{adjustbox}
\usepackage{wrapfig}
%\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{arydshln}

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[size=tiny]{todonotes}

\usepackage{microtype}

% This is also not strictly necessary, and may be commented out.
% However, it will improve the aesthetics of text in
% the typewriter font.
\usepackage{inconsolata}

%Including images in your LaTeX document requires adding
%additional package(s)
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage[noabbrev,capitalise]{cleveref}
\usepackage[normalem]{ulem}
\usepackage{comment}
\usepackage{pdfpages}
\usepackage{tabularx}
\usepackage{float}
\usepackage{array}
\usepackage{ragged2e}
\usepackage{placeins}

\usepackage{tcolorbox}  % For colored boxes
\usepackage{listings}   % For code formatting
\usepackage{tikz}       % TikZ package for drawing figures
\usepackage{geometry}   % To adjust the margins
%\usepackage{amsmath}    % For math symbols
\usepackage{pgfplots}   % For plots using PGFPlots
%\usepackage{graphicx}   % For including images
\usepackage{appendix}   % For creating the appendix
\usepackage{multicol}   % For multi-column layout
%\usepackage{float}      % To control float placement     


\newcommand{\cmark}{\textcolor{teal}{\textbf{{\checkmark}}}}  % Green checkmark
\newcommand{\xmark}{\textcolor{red}{\textbf{\texttimes}}}    % Red cross

% once finished, set all colors to black
\newcommand{\se}[1]{\textcolor{blue}{#1}}
\newcommand{\senew}[1]{\textcolor{blue}{#1}}
\newcommand{\leixin}[1]{\textcolor{blue}{#1}}
\newcommand{\cass}[1]{\textcolor{blue}{#1}}

\newcommand{\ourmodel}[0]{\texttt{ScImage}}
\newcommand{\dalle}[0]{\textsc{DALL·E}}
\newcommand{\automatikz}[0]{\textsc{AutomaTikZ}}
\newcommand{\llama}[0]{\textsc{Llama 3.1 8B}}
\newcommand{\gpt}[1]{\textsc{GPT-#1}}
\newcommand{\stablediffusion}[0]{\textsc{Stable Diffusion}}
\newcommand{\halfstar}{%
    \tikz[baseline=(star.base)]{
        \node[inner sep=0pt, outer sep=0pt] (star) {\faStar}; % Base full star
        \begin{scope}
            \clip (star.north west) -- (star.south west) -- (star.south) -- (star.north) -- cycle; % Clip left half
            \node[inner sep=0pt, outer sep=0pt, text=green] at (star.center) {\faStar}; % Overlay green on left half
        \end{scope}
    }%
}


\geometry{left=1in,right=1in,top=1in,bottom=1in}
\usepackage{caption}
\usepackage{array}

\lstdefinestyle{mystyle}{
    basicstyle=\ttfamily\footnotesize,
    breaklines=true,
    frame=single,
    backgroundcolor=\color{gray!10},
    keywordstyle=\color{blue},
    commentstyle=\itshape\color{green!50!black},
    showstringspaces=false
}

\lstset{style=mystyle, breaklines=true, breakatwhitespace=true}
% @@@@@@@@@@@@@@@@@@@@


\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\usepackage{fancyhdr} % Include the fancyhdr package

% \fancyhfoffset[L]{0pt} % Left header offset
\fancyhfoffset[R]{0pt} % Right header offset
%\iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.

==> latex/structure/guideline.tex <==
\section{Evaluation Guideline}\label{app:evaluation_guideline}
\subsection{Correctness}
\begin{table*}[htbp]
\small
\centering
\begin{tabularx}{\textwidth}{cX}
\toprule
\textbf{Score} & \textbf{Description} \\
\midrule
5 & The image fully meets all the requirements with no mistakes. \\
4 & The image meets the key requirements, with only minor mistakes. \\
3 & The image meets some or half of the requirements, with some mistakes. \\
2 & The image meets only a few of the text's requirements and contains serious mistakes. \\
1 & The image fails to meet the requirements of the text. \\
0 & No image content or compile error. \\
\bottomrule
\end{tabularx}
\caption{Correctness Scoring Guideline}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% table of examples
\begin{table*}[htbp]
\begin{tabularx}{\textwidth}{%
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X}

% First row: Images
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/1.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/2.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/3.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/4.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/5.png} \\[6pt]

{\centering
\small\textbf{Score:} 5\par} &
{\centering
\small\textbf{Score:} 4.2\par} &
{\centering
\small\textbf{Score:} 3\par} &
{\centering
\small\textbf{Score:} 2.4\par} &
{\centering
\small\textbf{Score:} 1.4\par} \\

% Second row: Prompts
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
\small There are 4 line segments inside a circle. 
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
The diagonal of the square is red and very thick. 
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
There are 5 squares on the left side of the canvas and 3 circles on the right side.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
The intersection of the circle and the square is filled with red.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
The intersection of the circle and the square is filled with red. 
\end{tabular}
\\

% Fourth row: Explanations
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
There are 4 line segments and they are inside a circle.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
The diagonal of the output image is not visibly very thick. Other than that it's correct.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
partially correct: The left graph shows a rectangle instead of 5 squares. The right-side graph is correct.
\end{tabular} &

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
The red-marked intersection does not involve a square. However, there is a red intersection and a circle.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
There is no square and no intersection of two graphs. (There is a circle and some red, but it’s overall incorrectly displayed).
\end{tabular}\\

\end{tabularx}
\caption{\textbf{Correctness Guideline Examples} \\ (Scores are averaged across multiple annotators)} 
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Relevance}
\begin{table*}[!t]
\small
\centering
\begin{tabularx}{\textwidth}{cX}
\toprule
\textbf{Score} & \textbf{Description} \\
\midrule
5 & The image contains no redundant objects or features. \\
4 & The image contains a few redundant objects or features but remains highly relevant to the text’s requirements. \\
3 & The image contains some redundant objects and some required elements. \\
2 & The image contains more redundant objects than required elements. \\
1 & The overall image is not relevant to the requirements. \\
0 & No image content or compile error. \\
\bottomrule
\end{tabularx}
\caption{Relevance Scoring Guideline}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\begin{tabularx}{\textwidth}{%
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X}

% First row: Images
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/1.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/2.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/3.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/4.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/5.png} \\[6pt]

{\centering
\small\textbf{Score:} 5\par} &
{\centering
\small\textbf{Score:} 4.6\par} &
{\centering
\small\textbf{Score:} 3.4\par} &
{\centering
\small\textbf{Score:} 2.2\par} &
{\centering
\small\textbf{Score:} 1.4\par} \\

% Second row: Prompts
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
\small The diagonal of the square is red.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
A binary tree with a total of 7 nodes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
The diagonal of the square is red and very thick.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
There are 4 tangent lines to a circle.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
There are 4 tangent lines to a circle.
\end{tabular}
\\

% Fourth row: Explanations
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
Fully relevant, no redundant objects or features.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
Additionally marked blue color for the tree nodes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
One redundant diagonal line in the square.
\end{tabular} &

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
A few redundant circles and two dotted straight lines. Additionally, there is a reddish color.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
Redundant curves inside the circle. Overall irrelevant image to the text. Also irrelevant coloring.
\end{tabular}\\

\end{tabularx}
\caption{\textbf{Relevence Guideline Examples} \\ (Scores are averaged across multiple annotators)} 
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Scientificness}
\begin{table*}[!t]
\small
\centering
\begin{tabularx}{\textwidth}{cX}
\toprule
\textbf{Score} & \textbf{Description} \\
\midrule
5 & The image can be presented in a textbook or academic paper without any change. \\
4 & The image has minor issues and requires minimal adjustments to be presented in a textbook or academic paper. \\
3 & The image has serious issues in scientific style, including mismatched sizes, unsuitable positions, overlapping graphs or text, incomplete graphs, etc. \\
2 & The image’s style is not common in scientific settings. \\
1 & The overall image is more suitable in a lifestyle context and is not appropriate for scientific demonstration. \\
0 & No image content or compile error. \\
\bottomrule
\end{tabularx}
\caption{Scientificness Quality Scoring Guideline}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[htbp]
\begin{tabularx}{\textwidth}{%
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X}

% First row: Images
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/1.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/2.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/3.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/4.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/5.png} \\[6pt]

{\centering
\small\textbf{Score:} 5\par} &
{\centering
\small\textbf{Score:} 4.2\par} &
{\centering
\small\textbf{Score:} 3.2\par} &
{\centering
\small\textbf{Score:} 1.8\par} &
{\centering
\small\textbf{Score:} 1.4\par} \\

% Second row: Prompts
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
\small A binary tree with a total of 7 nodes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
M triangles and N circles, where M is the same as N, and M and N are both larger than 2.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
Three triangles of the same size but different shapes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
A binary tree with a total of 7 nodes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
M triangles and N circles, where M is the same as N, and M and N are both larger than 2.
\end{tabular}
\\

% Fourth row: Explanations
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
perfect scientific image.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
A scientific image, but the triangles and circles are not arranged properly.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
There are many redundant lines around the triangles, which
negatively affects its demonstrative purpose.
\end{tabular} &

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
The representation of nodes and colorful edges are uncommon in
scientific images. Also, the quality (in terms of resolution) of the image is not what one would expect in modern science.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
The shapes are not strictly triangles and circles for scientific purposes. The image is closer to lifestyle. Also, the quality (in terms of resolution) of the image is not what one would expect in modern science.
\end{tabular}\\

\end{tabularx}
\caption{\textbf{Scientificness Guideline Examples} \\ (Scores are averaged across multiple annotators)} 
\end{table*}

==> latex/structure/table-example.tex <==
%\begin{table}[t!]
\begin{tabularx}{\textwidth}{|X|X|X|}
\hline
\textbf{Column 1} & \textbf{Column 2} & \textbf{Column 3} \\ \hline
This is a long text that adjusts to the column width. & Short text. & Another long text that adjusts dynamically. \\ \hline
More text. & Even more text. & Final column content. \\ \hline
\end{tabularx}
%\caption{Illustration of constructing generation queries.}
%\label{tab:prompt_template}
%\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> other_commands.tex <==
%\usepackage{xcolor}
\usepackage{fontawesome}
\usepackage{hyperref}
\usepackage{url}
\usepackage{times}
\usepackage{latexsym}
\usepackage{lscape}
\usepackage[export]{adjustbox}
%\usepackage[dvipsnames]{xcolor}

\usepackage{wrapfig}
%\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{graphicx}
%\usepackage{arydshln}

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[size=tiny]{todonotes}

\usepackage{microtype}

% This is also not strictly necessary, and may be commented out.
% However, it will improve the aesthetics of text in
% the typewriter font.
\usepackage{inconsolata}

%Including images in your LaTeX document requires adding
%additional package(s)
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage[noabbrev,capitalise]{cleveref}
\usepackage[normalem]{ulem}
\usepackage{comment}
\usepackage{pdfpages}
\usepackage{tabularx}
\usepackage{float}
\usepackage{array}
\usepackage{ragged2e}
\usepackage{placeins}

\usepackage{tcolorbox}  % For colored boxes
\usepackage{listings}   % For code formatting
\usepackage{tikz}       % TikZ package for drawing figures
\usepackage{geometry}   % To adjust the margins
%\usepackage{amsmath}    % For math symbols
\usepackage{pgfplots}   % For plots using PGFPlots
%\usepackage{graphicx}   % For including images
\usepackage{appendix}   % For creating the appendix
\usepackage{multicol}   % For multi-column layout
%\usepackage{float}      % To control float placement     


\newcommand{\cmark}{\textcolor{teal}{\textbf{{\checkmark}}}}  % Green checkmark
\newcommand{\xmark}{\textcolor{red}{\textbf{\texttimes}}}    % Red cross

% once finished, set all colors to black
\newcommand{\se}[1]{\textcolor{blue}{#1}}
\newcommand{\senew}[1]{\textcolor{blue}{#1}}
\newcommand{\leixin}[1]{\textcolor{blue}{#1}}
\newcommand{\cass}[1]{\textcolor{blue}{#1}}

\newcommand{\ourmodel}[0]{\texttt{ScImage}}
\newcommand{\dalle}[0]{\textsc{DALL·E}}
\newcommand{\automatikz}[0]{\textsc{AutomaTikZ}}
\newcommand{\llama}[0]{\textsc{Llama 3.1 8B}}
\newcommand{\gpt}[1]{\textsc{GPT-#1}}
\newcommand{\stablediffusion}[0]{\textsc{Stable Diffusion}}
\newcommand{\halfstar}{%
    \tikz[baseline=(star.base)]{
        \node[inner sep=0pt, outer sep=0pt] (star) {\faStar}; % Base full star
        \begin{scope}
            \clip (star.north west) -- (star.south west) -- (star.south) -- (star.north) -- cycle; % Clip left half
            \node[inner sep=0pt, outer sep=0pt, text=green] at (star.center) {\faStar}; % Overlay green on left half
        \end{scope}
    }%
}


\geometry{left=1in,right=1in,top=1in,bottom=1in}
\usepackage{caption}
\usepackage{array}

\lstdefinestyle{mystyle}{
    basicstyle=\ttfamily\footnotesize,
    breaklines=true,
    frame=single,
    backgroundcolor=\color{gray!10},
    keywordstyle=\color{blue},
    commentstyle=\itshape\color{green!50!black},
    showstringspaces=false
}

\lstset{style=mystyle, breaklines=true, breakatwhitespace=true}
% @@@@@@@@@@@@@@@@@@@@


\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\usepackage{fancyhdr} % Include the fancyhdr package

% \fancyhfoffset[L]{0pt} % Left header offset
\fancyhfoffset[R]{0pt} % Right header offset
\iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.

==> other_commands_orig.tex <==
%\usepackage{xcolor}
\usepackage{fontawesome}
\usepackage{hyperref}
\usepackage{url}
\usepackage{times}
\usepackage{latexsym}
\usepackage{lscape}
\usepackage[dvipsnames]{xcolor}
\usepackage[export]{adjustbox}
\usepackage{wrapfig}
%\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{arydshln}

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[size=tiny]{todonotes}

\usepackage{microtype}

% This is also not strictly necessary, and may be commented out.
% However, it will improve the aesthetics of text in
% the typewriter font.
\usepackage{inconsolata}

%Including images in your LaTeX document requires adding
%additional package(s)
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage[noabbrev,capitalise]{cleveref}
\usepackage[normalem]{ulem}
\usepackage{comment}
\usepackage{pdfpages}
\usepackage{tabularx}
\usepackage{float}
\usepackage{array}
\usepackage{ragged2e}
\usepackage{placeins}

\usepackage{tcolorbox}  % For colored boxes
\usepackage{listings}   % For code formatting
\usepackage{tikz}       % TikZ package for drawing figures
\usepackage{geometry}   % To adjust the margins
%\usepackage{amsmath}    % For math symbols
\usepackage{pgfplots}   % For plots using PGFPlots
%\usepackage{graphicx}   % For including images
\usepackage{appendix}   % For creating the appendix
\usepackage{multicol}   % For multi-column layout
%\usepackage{float}      % To control float placement     


\newcommand{\cmark}{\textcolor{teal}{\textbf{{\checkmark}}}}  % Green checkmark
\newcommand{\xmark}{\textcolor{red}{\textbf{\texttimes}}}    % Red cross

% once finished, set all colors to black
\newcommand{\se}[1]{\textcolor{blue}{#1}}
\newcommand{\senew}[1]{\textcolor{blue}{#1}}
\newcommand{\leixin}[1]{\textcolor{blue}{#1}}
\newcommand{\cass}[1]{\textcolor{blue}{#1}}

\newcommand{\ourmodel}[0]{\texttt{ScImage}}
\newcommand{\dalle}[0]{\textsc{DALL·E}}
\newcommand{\automatikz}[0]{\textsc{AutomaTikZ}}
\newcommand{\llama}[0]{\textsc{Llama 3.1 8B}}
\newcommand{\gpt}[1]{\textsc{GPT-#1}}
\newcommand{\stablediffusion}[0]{\textsc{Stable Diffusion}}
\newcommand{\halfstar}{%
    \tikz[baseline=(star.base)]{
        \node[inner sep=0pt, outer sep=0pt] (star) {\faStar}; % Base full star
        \begin{scope}
            \clip (star.north west) -- (star.south west) -- (star.south) -- (star.north) -- cycle; % Clip left half
            \node[inner sep=0pt, outer sep=0pt, text=green] at (star.center) {\faStar}; % Overlay green on left half
        \end{scope}
    }%
}


\geometry{left=1in,right=1in,top=1in,bottom=1in}
\usepackage{caption}
\usepackage{array}

\lstdefinestyle{mystyle}{
    basicstyle=\ttfamily\footnotesize,
    breaklines=true,
    frame=single,
    backgroundcolor=\color{gray!10},
    keywordstyle=\color{blue},
    commentstyle=\itshape\color{green!50!black},
    showstringspaces=false
}

\lstset{style=mystyle, breaklines=true, breakatwhitespace=true}
% @@@@@@@@@@@@@@@@@@@@


\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\usepackage{fancyhdr} % Include the fancyhdr package

% \fancyhfoffset[L]{0pt} % Left header offset
\fancyhfoffset[R]{0pt} % Right header offset
%\iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.

==> structure/analysis.tex <==
\section{Analysis}

We conduct a more detailed analysis of model performance, focusing on understanding types (attribute, numerical and spatial understanding) and object types to identify which categories present the greatest challenges for the models.


\paragraph{Types of Understanding} 
\cref{tab:understanding_with_0} presents 
the fine-grained correctness scores for different understanding types. Figure \ref{fig:understanding_type_with_0} illustrates the performance of two modes of generation (text-code-image and text-image) separately. Notably, spatial understanding appears to be the most challenging across all textual models. For instance, while \gpt{4o} achieves scores around 4.0 for attribute binding, its performance drops %significantly 
substantially for spatial understanding, remaining well below 3.5.



\begin{wrapfigure}{hr}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{latex/plots/understanding_type.pdf}
    \caption{Comparison of text-code-image and text-image: 
    correctness scores, averaged across model types, of each understanding %type. 
    category. 
    `Three types' means
    attribute, numerical and spatial understanding combined.}
    \label{fig:understanding_type_with_0}
\vspace{-20pt}
\end{wrapfigure}
%Among the three reasoning types—spatial reasoning, numerical reasoning, and attribute binding—spatial reasoning is the most challenging for all textual generation models. 
%Their code-converted images consistently receive the lowest correctness scores compared to their average performance in numerical understanding and attribute binding. 
%For example, \texttt{GPT-4o} images achieve average scores of approximately 4.0 or higher for numerical understanding and attribute binding converted from TikZ and Python-generated code, while its spatial reasoning score is lower, at 3.82.
% For example, \gpt{4o} achieves scores of about 4 for understanding but clearly below 3.5 for spatial understanding. \llama{} with Python output has the largest discrepancy between numeric (3.72) and spatial (2.5) understanding. 


In contrast, for the image generation models %like %\texttt{Stable Diffusion} 
\stablediffusion{}
and %\texttt{DALL·E}, 
\dalle{}, 
numerical comprehension poses the greatest challenge (\cref{fig:understanding_type_with_0}). Both models score between %1.7 and 
below 1.8 for numerical understanding, substantially lower than their scores for attribute understanding %(2.75 for \texttt{Stable Diffusion} 
($\sim$2.7)
%and 2.68 for \texttt{DALL·E}) 
and spatial understanding %(2.06 and 2.13, respectively).
(above 2.0). This indicates an interesting discrepancy between model types.

Due to their weakness in spatial understanding, tasks that involve combined understanding types—including numerical \& spatial understanding, as well as numerical \&  spatial \&  attribute understanding—also tend to receive lower scores. Both \gpt{4o}\_python and \gpt{4o}\_tikz record their lowest scores when addressing prompts that require all three understanding types, in comparison to prompts focused on individual understanding types.


\begin{table}[!t]
\centering
\small
\resizebox{0.8\textwidth}{!}
{\begin{tabular}{rccccccc}
\hline
\textbf{Model}   & {\color[HTML]{333333} \textbf{Attribute}} & {\color[HTML]{333333} \textbf{Numerical}} & {\color[HTML]{333333} \textbf{Spatial}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Attribute \&\\ Numerical\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Attribute \&\\ Spatial\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Numerical \&\\ Spatial\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Attribute \&\\ Numerical \& \\Spatial\end{tabular}}\\ \hline
Automatikz       & 2.42               & 1.91               & 1.71             & 2.29                   & 2.04                  & 2.13                 & 1.77                              \\
Llama\_tikz      & 2.53               & 1.55               & 1.77             & 1.69                   & 1.84                  & 1.91                 & 1.3                               \\
GPT-4o\_tikz     & 4.11               & 3.49               & 3.35             & 3.41                   & 3.53                  & 3.59                 & 3.13                              \\
Llama\_python    & 2.24               & 2.38               & 1.96             & 2.28                   & 2.28                  & 1.63                 & 1.97                              \\
GPT-4o\_python   & 3.95               & 3.92               & 3.47             & 3.46                   & 3.34                  & 3.28                 & 3.13                              \\
Stable Diffusion & 2.75               & 1.73               & 2.06             & 2.41                   & 2.46                  & 1.96                 & 2.11                              \\
DALL ·E          & 2.68               & 1.77               & 2.13             & 2.36                   & 2.31                  & 1.94                 & 2.07                             \\ %\cdashline{1-8}
Average &2.95	
&2.39	&2.35&	2.56&	2.54	&2.35&	2.21\\ \hline
Sample Size & 48 & 64 & 56 & 80 & 40 & 64 & 52 \\ \hline
\end{tabular}
}
\caption{Correctness evaluation within each understanding category (compile errors are penalized with score 0). }
\label{tab:understanding_with_0}
\end{table}

\paragraph{Object Categories} 

% We classify the object complexity of all prompts based on object types and calculate the average scores for each category, specifically: 2D geometric shapes, 3D geometric shapes, charts, graph theory representations, matrices, real-life object modeling, tables, additional annotations, functions, and coordinates.





\begin{table*}[!h]
\centering
\resizebox{0.88\textwidth}{!}
{
\begin{tabular}{rccccccccc}
\hline
\textbf{Model}            & \textbf{2D shape}                          & \textbf{3D shape}                          & \textbf{Chart}                       & \textbf{\begin{tabular}[c]{@{}c@{}}Graph theory\end{tabular}}                        & \textbf{Matrix}                      & \textbf{\begin{tabular}[c]{@{}c@{}}Real-life object\end{tabular}} & \textbf{Table}                       & \textbf{\begin{tabular}[c]{@{}c@{}}Annotation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Function\&\\ Coordinate\end{tabular}} \\ \hline
Automatikz       & 2.50               & 1.52               & 1.71             & 2.40                   & 1.81                  & 1.89                 & 2.13                              & 1.33                 & 1.90                 \\
Llama\_tikz      & 2.72               & 1.45               & 0.47             & 0.10                   & 2.06                  & 1.42                 & 1.13                              & 1.33                 & 1.55                 \\
GPT-4o\_tikz     & 3.90               & 3.19               & 3.12             & 3.63                   & 3.00                  & 3.14                 & 4.38                              & 3.56                 & 3.45                 \\
Llama\_python    & 2.49               & 1.39               & 3.15             & 0.00                   & 0.94                  & 2.37                 & 0.00                              & 2.00                 & 2.13                 \\
GPT-4o\_python   & 4.05               & 3.11               & 3.25             & 2.73                   & 3.13                  & 3.25                 & 3.88                              & 3.39                 & 3.20                 \\
Stable Diffusion & 2.08               & 2.43               & 2.11             & 1.43                   & 1.56                  & 2.96                 & 2.13                              & 2.11                 & 1.75                 \\
DALL ·E          & 2.08               & 2.47               & 1.86             & 1.25                   & 1.50                  & 3.17                 & 1.75                              & 2.11                 & 1.58       \\ 
%\cdashline{1-10}
{Average} & 2.83                 & 2.22               & 2.24                      & 1.65                 & 2.00               & 2.60                 & 2.20                 & 2.26               & 2.22                      \\ \hline
Sample Size & 162 & 97 & 54 & 20 & 8 & 38 & 4 & 9 & 20 \\ \hline
\end{tabular}
}
\caption{Object Complexity for Models: Correctness scores by object type.}
\label{tab:object_with_0}
\end{table*}

Table \ref{tab:object_with_0} presents the average correctness scores for each object category. The performance of different model types (Text-TikZ-Image, Text-Python-Image, and Text-Image) is visualized separately in \cref{fig:object_complex_radar_with_0}. In general, graph theory representation (e.g. nodes and edges in a binary tree or graph) poses great challenges for models, with an average score below 1.7 across all models, compared to above 2.0 the remaining object categories. 

As illustrated in \cref{fig:object_complex_radar_with_0}, \gpt{4o} is the top-performing model across all object types, with both TikZ and Python-generated images consistently achieving the highest scores within each category. However, \gpt{4o} shows slightly lower performance in generating matrices (TikZ score: 3.00), 3D shapes (Python score: 3.11), and real-life object models (TikZ score: 3.14).






\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.85\textwidth]{latex/plots/radar_charts_same_scale_1.pdf}
    \caption{Generation performance of models on different object types. The same scale is used for three radar bars, with the center as correctness score 0, and the outermost circle as 5.}
    \label{fig:object_complex_radar_with_0}
\end{figure*}

% Its TikZ output outperforms its Python code in 6 out of 9 object types. Notably, \texttt{GPT-4o\_tikz} excels in graph theory representations (4.26), charts (4.11), 2D geometric shapes (4.13), and matrices (4.00). However, \texttt{GPT-4o\_python} performs better than \texttt{GPT-4o\_tikz} for 2D geometric shapes (4.28), 3D shapes (3.47), and real-life object modeling (3.42).


% , but worse for real-life object modeling (3.28), tables (3.56), functions and coordinates (3.63), and 3D geometric shapes. 

% Its scores for functions and coordinates (3.20), charts (3.31), and tables (3.25) are lower than its tikz code converted counterparts.


%\textbf{Llama-3.1-8B}: 
%\llama{}:
%Among all object types, 
\llama{} (in both TikZ and Python code) clearly struggles with the representation of graph theory structures, such as nodes and edges, with a correctness score close to 0. Similarly, it performs poorly in table generation, scoring 1.13 with TikZ and 0 with Python. The largest discrepancy between TikZ and Python output is observed in chart generation, where TikZ achieves a score of 0.47, while Python scores 3.15. In contrast, TikZ outperforms Python in matrix generation, with correctness scores of 2.06 and 0.94, respectively. This may be attributed to the availability of libraries with Python and TikZ code. Matplotlib in Python is frequently used for chart and plot representation, while the usage of matrix presentation with proper math format is rare.

% \todo{SE: what are the scales in Fig. 4? Can we compare all three images? Image is changed to the same scale}

% Among all object types, \texttt{Llama\_tikz} code performs best when generating 2D geometric shapes (3.10), while \texttt{Llama\_python} code excels in chart generation (3.95), the type \texttt{Llama\_tikz} struggles with at 1.96. Both methods—TikZ and Python code to image—perform worst for graph theory representations, such as binary trees or node-and-edge diagrams, with \texttt{Llama\_tikz} scoring 1.00 and \texttt{Llama\_python} scoring 0, as no image could be compiled from the generated Python code.



\begin{table*}[t!]
\small
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{r|cccc|cccc|cccc}
\hline
\textbf{Criteria}          & \multicolumn{4}{c|}{\textbf{Correctness}}                     & \multicolumn{4}{c|}{\textbf{Relevance}}                       & \multicolumn{4}{c}{\textbf{Scientific style}}                \\ \hline
{Language}       & EN            & DE            & ZH            & FA            & EN            & DE            & ZH            & FA            & EN            & DE            & ZH            & FA            \\ \hline
{Llama\_tikz}    & {1.88} & 1.48          & 1.50          & 1.23          & {2.18} & 1.78          & 2.10          & 1.68          & 2.78          & 2.23          & 2.80          & {2.90} \\
{GPT-4o\_tikz}   & 3.85          & {4.03} & {3.98} & {3.68} & {4.03} & 4.23          & {4.60} & {3.98} & {4.10} & {4.43} & 4.40          & 3.98          \\
{OpenAI-o1\_tikz}   & {4.43} & 3.68          & 3.83          & 4.05          & {4.45} & 3.80          & 4.10          & 4.18          & {4.40} & 3.88          & 4.03          & 4.05          \\
{Llama\_python}  & {2.53} & {1.35} & 1.75          & 1.78          & {2.70} & {1.53} & 2.00          & {1.90} & 3.20          & 2.50          & 3.10          & {3.30} \\
{GPT-4o\_python} & 3.38          & {4.15} & 4.13          & 3.48          & 3.35          & 4.18          & {4.23} & 3.35          & 3.88          & 4.50          & {4.83} & 3.85          \\
{OpenAI-o1\_python} & {4.28} & 3.45          & 4.10          & 3.60          & {4.10} & 3.45          & 3.93          & 3.60          & {4.50} & 4.08          & 4.30          & 4.05          \\
DALL-E                  & 1.98          & {2.15} & 1.83          & 1.93          & 1.88          & {2.03} & {2.03} & 2.00          & 1.40          & {1.58} & 1.53          & 1.50          \\ %\cdashline{1-13}
Average        & {3.19}  & 2.90           & 3.01           & 2.82           & 3.24           & 3.00           & {3.28} & 2.95          & 3.46             & 3.31            & {3.57}   & 3.38            \\ \hline
\end{tabular}
}
\caption{Multilingual performance of overall generations.}
\label{tab:multilingual_with_0}
\end{table*}



% \begin{wrapfigure}{l}{0.45\textwidth}
%     \centering
%     \includegraphics[width=0.45\textwidth]{multilingual_e2326.pdf}
%     \caption{Multilingual Performance of Models (scores averaged across models)}
%     \label{fig:multilingual}
% \end{wrapfigure}

 %\texttt{Automatikz} 

\automatikz{} 
shows the lowest scores for annotation (1.33) and 3D geometric shape generation (1.52) across all object types. It performs best in 2D geometric shape generation (2.52), though it still lags behind %\texttt{GPT-4o} and \texttt{llama}, 
\gpt{4o}, 
which scores above 3.  %\texttt{Stable Diffusion} and \texttt{DALL·E} 






\cref{fig:object_complex_radar_with_0} reveals that code-generated images are of higher quality for 2D geometric shapes compared to 3D shapes, while visual models exhibit the opposite trend. \stablediffusion{} and \dalle{} 
perform best in real-life object modeling, with scores of 3.12 and 3.24, respectively, and in 3D geometric shape generation, with scores of 2.43 and 2.47. %\todo{SE: I feel real-life object modeling is a bit underdefined}






\paragraph{Multilingual Evaluation} %The purpose of the multilingual experiments is to 
We further evaluate model performance across diverse languages. %building on prior testing conducted in English. 
Due to the high annotation costs, we sample 20 instructions and translate them into Chinese, German and Farsi by native language co-authors. 
Each prompt is derived from a unique template to ensure diversity. %in prompts. 
% \todo{SE: is that true? Leixin: Yes}
Moreover, these instructions are %meticulously 
curated to encompass all %comprehensive 
understanding dimensions: the single dimension of spatial, attribute, or numerical understanding; combinations of two dimensions (e.g., prompts requiring both attribute and numerical understanding); and prompts requiring all three understanding dimensions. We then feed the 20 prompts to all models except for \automatikz{}, which is our only model fine-tuned on English TikZ data, and \stablediffusion{}. We additionally include the very recently released OpenAI o1-preview here, which focuses on science, coding, and math \citep{openai_o1_preview}.  


Results are shown in Table \ref{tab:multilingual_with_0}. Interestingly, English does not always lead to best results on average. While correctness is highest with English prompts with a margin of 0.18 ahead of Chinese,  outputs generated from Chinese prompts are better according to relevance and scientificness. Farsi is worst on average. Among models, \llama{} becomes considerably worse regarding correctness and relevance in languages other than English, while \gpt{4o} %is often at least as good in other languages as in English. %
often even performs better in non-English languages.
%However, it is interesting that 
Remarkably, 
OpenAI o1-preview is better than \gpt{4o} in English (and regarding its maximum scores), often by a considerable margin (e.g., 4.28 vs.\ 3.38 in correctness for English input with python output), but performs substantially worse in non-English languages (e.g., 3.45 vs.\ 4.15 in German with python output), except for Farsi. 



\begin{wraptable}{l}{0.5\textwidth}
\small
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{rcccc}
\hline
\textbf{Code} & \textbf{Correctness} & \textbf{Relevance} & \textbf{Scientific style} &\textbf{Error rate} \\ \hline
TikZ          & 2.64                 & 2.81               & 3.18  &                   0.19 \\
Python        & 2.81                 & 2.97               & 3.56    & 0.17                  \\ \hline
\end{tabular}}
\caption{Comparison of TikZ code performance and Python code performance: scores averaged from model \gpt{4o} and \llama{}. Compile errors are penalized with a score 0.}
\label{tab:tikz_python_with_0}
\vspace{-20pt}
\end{wraptable}

\paragraph{Output code difference} As shown in \cref{tab:tikz_python_with_0}, Python code generation outperforms TikZ output across all three evaluation criteria: Correctness, Relevance and Scientific style. Furthermore, the Python code output exhibits a lower compile error rate (0.17 for Python vs. 0.19 for TikZ). The disparity may be attributed to the richer resources of available Python code in the training data for LLMs. 



\paragraph{Qualitative Analysis}
We diagnose some issues by closely examining the generated output images, specifically highlighting problems that point to areas for future improvement in the models. For instance, the generated images from some models reveal a lack of physics knowledge. In cases requiring an image of liquid in a container (\cref{fig:wrong_examples}), the liquid is often placed incorrectly, not at the bottom of the container. This issue occasionally occurs with %\texttt{automatikz}, 
\automatikz{} and \llama{}, 
but it is not observed in models like %\texttt{GPT-4o}, \texttt{Stable Diffusion}, or \texttt{DALL·E}.
\gpt{4o}, \stablediffusion{} and \dalle{}. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{latex/plots/wrong_examples_2.pdf}
    \caption{Incorrect output from models %for the 
    arguably due to a 
    lack of world knowledge}
    \label{fig:wrong_examples}
\end{figure}

%\todo{SE: how does 'a liquid filled with a container' fit into our scheme? Liquid and container are objects from Datikz? What are spatial, attribute and numeric dimension here?}

A challenging scenario for most models is generating an object moving along a parabolic path. \gpt{4o} and \llama{} 
occasionally depict a correct downward-opening parabola, but upward-opening parabolas also exist in their generation, indicating a lack of understanding of the trajectory of how an object moves. 
Another common issue across models is their difficulty in generating images that depict ``boxes placed on a slope at a specific angle''. Although \gpt{4o} sometimes manages to generate the correct image, their performance is inconsistent. This suggests a lack of understanding of the interaction between gravity and the support surface, as well as difficulty positioning objects at the correct angle on a 2D plane. 

% \todo{SE: I am not so sure I like this annalysis. Could we quantitatively identify some images that are bad by all models?}

% Moreover, \gpt{4o} exhibits a significant issue in code generation: It frequently copies parts of the code from previous generations to a new prompt requirement. This leads to overlapped graphs.  \todo{SE: this is our bug --- not sure if it is clever to mention this explicitly}

% \todo[inline]{SE: which spatial/attribute/numeric dimension is covered in "a container is filled with water"? Spatial --- filled with? The caption was simplified, should be 'spatial' + 'numerical' of water amount. The full prompts are added}

%\input{latex/structure/metrics}

==> structure/conclusion.tex <==
\section{Concluding remarks}\label{sec:conclusion}


Our study presents the first comprehensive evaluation of multimodal LLMs for scientific image generation, using %the 
our novel \ourmodel{} benchmark. Our assessment reveals both significant progress and persistent challenges in the field. While models like %GPT4-o 
\gpt{4o}
sometimes demonstrate proficiency in tasks involving individual dimensions of understanding (spatial, numeric, or attribute-based in isolation), all evaluated models struggle with complex tasks requiring combined understanding. On average, even \gpt{4o} performs below 4 on correctness on our benchmark. For example, due to its lack of world knowledge or an inability to correctly plan how a 3D object should be presented, GPT4 sometimes has difficulty arranging objects correctly in a two-dimensional image. Code based models have difficulties especially with spatial understanding, while image based models struggle the most with numeric understanding.

We find that code-based outputs generally outperform direct image generation in producing scientifically styled images. However, %spatial understanding remains a significant challenge across all models, particularly when combined with other types of comprehension. P
performance varies considerably across different object types and languages, highlighting the need for more robust and consistent modeling approaches in the scientific domain. These findings underscore the importance of continued research to enhance multimodal LLMs' capabilities in scientific image generation. By providing a standardized benchmark and detailed analysis, \ourmodel{} aims to drive progress in this critical area, supporting more efficient scientific communication and accelerating cross-disciplinary research.

As multimodal LLMs evolve, their potential to revolutionize scientific content generation 
remains an exciting frontier in AI research. Future work should focus on improving models' ability to handle complex, multi-dimensional reasoning tasks and ensure consistent performance across diverse scientific domains and languages. As science serves humanity and should be accessible by everyone to foster diversity and inclusion, this concerns particularly \emph{open-source} models which can be considered at best mediocre for the tasks sketched in \ourmodel{}, with performances that substantially lag behind closed-source proprietary models like \gpt{4}. 







==> structure/experiments.tex <==









\begin{comment}
    

\begin{itemize}
    \item 1) We construct a taxonomy suitable for text-image understanding (based on what?)
    \item 2) We build a dataset of pairs of captions and reference images. The dataset includes 0,1,2,... reference images per caption. How? 
    \item 3) We apply several multimodal models on our dataset to test their scientific text-to-image conversion abilities/understanding
    \item 4) We use human eval and automatic metrics
    \item 5) Optionally: we fine-tune automatikz on our dataset
\end{itemize}                                                                                          
Instantiation of 1) below:

In a scientific graph containing a single object, such as a circle or a square, we assume that the image meets the requirements of the caption if the following factors are well-controlled:
\begin{itemize}

    \item \textbf{Object}: Ensuring the shape is accurately represented according to the scientific standards required.
    \item \textbf{Properties of Objects}: includes colour, line or contour, size, and other relevant physical attributes. Additionally, the object may be subject to operations such as rotation or flipping to enhance clarity or emphasis. 
    \item \textbf{Position} of the object in the image
\end{itemize}

In a word, a correct scientific graph with a single object should meet the shape × properties × position requirement. 

The types of objects include geometric shapes, including those of 2 dimensions e.g. square or perpendicular, and also those in 3 dimensional space like a sphere. They can also be specific to a particular field or discipline. [UNFINISHED PARAGRAPH]

Composition: For graphs that combine two or more objects, the number of objects, their arrangement (the way of composition), and their comparative properties are crucial for accurate scientific representation. The way of composition may include the following examples.
\begin{itemize}
    \item Two triangles\textbf{ share the same side}.
    \item Two lines \textbf{perpendicular or parallel} to each other.
    \item Five circles with the \textbf{same centre} (five \textbf{concentric} circles).
    \item Three circles \textbf{without intersecting}.
\end{itemize}


\textbf{Annotation}: Additionally, annotations are often necessary to provide clarity or emphasize specific features. These may include textual annotations, for instance: text \texttt{`Linear Function: $y=3x$'} for its function graph, or the annotation of `A', `B' and `C' in the following example: \texttt{C is the midpoint of line AB}. Numerical annotations are also useful, for instance, in labeling the values on a bar chart. Additionally, scientific graphs may incorporate symbols or arrows to highlight or direct attention to particular segments or details of the graph."




\subsection{Evaluation Dataset SciGra (temperate dataset name)}

To investigate VLLMs' capability of generating scientific graphs, we create an evaluation dataset, SciGra. SciGra contains xxx prompts that instruct the VLLM model to generate scientific graphs. SciGra also provides a reference graph and an attribute set (e.g. number and color) for each prompt. Table xx shows a subset of SciGra.

\newline
[Table shows 1-2 examples]
\newline

\paragraph{Checklist} How we create attributes

\paragraph{Prompt Template}


\subsection{Human Evaluation}



\subsection{Automatic Evaluation}





\begin{itemize}
    \item 1) We construct a taxonomy suitable for text-image understanding (based on what?)
    \item 2) We build a dataset of pairs of captions and reference images. The dataset includes 0,1,2,... reference images per caption. How? 
    \item 3) We apply several multimodal models on our dataset to test their scientific text-to-image conversion abilities/understanding
    \item 4) We use human eval and automatic metrics
    \item 5) Optionally: we fine-tune automatikz on our dataset
\end{itemize}                                                                                          
Instantiation of 1) below:

In a scientific graph containing a single object, such as a circle or a square, we assume that the image meets the requirements of the caption if the following factors are well-controlled:
\begin{itemize}

    \item \textbf{Object}: Ensuring the shape is accurately represented according to the scientific standards required.
    \item \textbf{Properties of Objects}: includes colour, line or contour, size, and other relevant physical attributes. Additionally, the object may be subject to operations such as rotation or flipping to enhance clarity or emphasis. 
    \item \textbf{Position} of the object in the image
\end{itemize}

In a word, a correct scientific graph with a single object should meet the shape × properties × position requirement. 

The types of objects include geometric shapes, including those of 2 dimensions e.g. square or perpendicular, and also those in 3 dimensional space like a sphere. They can also be specific to a particular field or discipline. [UNFINISHED PARAGRAPH]

Composition: For graphs that combine two or more objects, the number of objects, their arrangement (the way of composition), and their comparative properties are crucial for accurate scientific representation. The way of composition may include the following examples.
\begin{itemize}
    \item Two triangles\textbf{ share the same side}.
    \item Two lines \textbf{perpendicular or parallel} to each other.
    \item Five circles with the \textbf{same centre} (five \textbf{concentric} circles).
    \item Three circles \textbf{without intersecting}.
\end{itemize}

\end{comment}


==> structure/guideline.tex <==
\section{Evaluation Guideline}\label{app:evaluation_guideline}
\subsection{Correctness}
\begin{table*}[htbp]
\small
\centering
\begin{tabularx}{\textwidth}{cX}
\toprule
\textbf{Score} & \textbf{Description} \\
\midrule
5 & The image fully meets all the requirements with no mistakes. \\
4 & The image meets the key requirements, with only minor mistakes. \\
3 & The image meets some or half of the requirements, with some mistakes. \\
2 & The image meets only a few of the text's requirements and contains serious mistakes. \\
1 & The image fails to meet the requirements of the text. \\
0 & No image content or compile error. \\
\bottomrule
\end{tabularx}
\caption{Correctness Scoring Guideline}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% table of examples
\begin{table*}[htbp]
\begin{tabularx}{\textwidth}{%
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X}

% First row: Images
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/1.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/2.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/3.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/4.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/correctness/5.png} \\[6pt]

{\centering
\small\textbf{Score:} 5\par} &
{\centering
\small\textbf{Score:} 4.2\par} &
{\centering
\small\textbf{Score:} 3\par} &
{\centering
\small\textbf{Score:} 2.4\par} &
{\centering
\small\textbf{Score:} 1.4\par} \\

% Second row: Prompts
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
\small There are 4 line segments inside a circle. 
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
The diagonal of the square is red and very thick. 
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
There are 5 squares on the left side of the canvas and 3 circles on the right side.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
The intersection of the circle and the square is filled with red.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
The intersection of the circle and the square is filled with red. 
\end{tabular}
\\

% Fourth row: Explanations
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
There are 4 line segments and they are inside a circle.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
The diagonal of the output image is not visibly very thick. Other than that it's correct.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
partially correct: The left graph shows a rectangle instead of 5 squares. The right-side graph is correct.
\end{tabular} &

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
The red-marked intersection does not involve a square. However, there is a red intersection and a circle.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
There is no square and no intersection of two graphs. (There is a circle and some red, but it’s overall incorrectly displayed).
\end{tabular}\\

\end{tabularx}
\caption{\textbf{Correctness Guideline Examples} \\ (Scores are averaged across multiple annotators)} 
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Relevance}
\begin{table*}[!t]
\small
\centering
\begin{tabularx}{\textwidth}{cX}
\toprule
\textbf{Score} & \textbf{Description} \\
\midrule
5 & The image contains no redundant objects or features. \\
4 & The image contains a few redundant objects or features but remains highly relevant to the text’s requirements. \\
3 & The image contains some redundant objects and some required elements. \\
2 & The image contains more redundant objects than required elements. \\
1 & The overall image is not relevant to the requirements. \\
0 & No image content or compile error. \\
\bottomrule
\end{tabularx}
\caption{Relevance Scoring Guideline}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\begin{tabularx}{\textwidth}{%
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X}

% First row: Images
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/1.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/2.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/3.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/4.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/relevence/5.png} \\[6pt]

{\centering
\small\textbf{Score:} 5\par} &
{\centering
\small\textbf{Score:} 4.6\par} &
{\centering
\small\textbf{Score:} 3.4\par} &
{\centering
\small\textbf{Score:} 2.2\par} &
{\centering
\small\textbf{Score:} 1.4\par} \\

% Second row: Prompts
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
\small The diagonal of the square is red.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
A binary tree with a total of 7 nodes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
The diagonal of the square is red and very thick.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
There are 4 tangent lines to a circle.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
There are 4 tangent lines to a circle.
\end{tabular}
\\

% Fourth row: Explanations
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
Fully relevant, no redundant objects or features.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
Additionally marked blue color for the tree nodes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
One redundant diagonal line in the square.
\end{tabular} &

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
A few redundant circles and two dotted straight lines. Additionally, there is a reddish color.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
Redundant curves inside the circle. Overall irrelevant image to the text. Also irrelevant coloring.
\end{tabular}\\

\end{tabularx}
\caption{\textbf{Relevence Guideline Examples} \\ (Scores are averaged across multiple annotators)} 
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Scientificness}
\begin{table*}[!t]
\small
\centering
\begin{tabularx}{\textwidth}{cX}
\toprule
\textbf{Score} & \textbf{Description} \\
\midrule
5 & The image can be presented in a textbook or academic paper without any change. \\
4 & The image has minor issues and requires minimal adjustments to be presented in a textbook or academic paper. \\
3 & The image has serious issues in scientific style, including mismatched sizes, unsuitable positions, overlapping graphs or text, incomplete graphs, etc. \\
2 & The image’s style is not common in scientific settings. \\
1 & The overall image is more suitable in a lifestyle context and is not appropriate for scientific demonstration. \\
0 & No image content or compile error. \\
\bottomrule
\end{tabularx}
\caption{Scientificness Quality Scoring Guideline}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[htbp]
\begin{tabularx}{\textwidth}{%
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X
    >{\RaggedRight\arraybackslash}X}

% First row: Images
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/1.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/2.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/3.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/4.png} &
\includegraphics[width=\linewidth]{latex/plots/guideline/scientific/5.png} \\[6pt]

{\centering
\small\textbf{Score:} 5\par} &
{\centering
\small\textbf{Score:} 4.2\par} &
{\centering
\small\textbf{Score:} 3.2\par} &
{\centering
\small\textbf{Score:} 1.8\par} &
{\centering
\small\textbf{Score:} 1.4\par} \\

% Second row: Prompts
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
\small A binary tree with a total of 7 nodes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
M triangles and N circles, where M is the same as N, and M and N are both larger than 2.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
Three triangles of the same size but different shapes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
A binary tree with a total of 7 nodes.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Prompt:} \\[6pt]
M triangles and N circles, where M is the same as N, and M and N are both larger than 2.
\end{tabular}
\\

% Fourth row: Explanations
\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
perfect scientific image.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
A scientific image, but the triangles and circles are not arranged properly.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
There are many redundant lines around the triangles, which
negatively affects its demonstrative purpose.
\end{tabular} &

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
The representation of nodes and colorful edges are uncommon in
scientific images. Also, the quality (in terms of resolution) of the image is not what one would expect in modern science.
\end{tabular}&

\begin{tabular}[t]{@{}p{\linewidth}@{}}
\justify
\small\textbf{Explanation:} \\[6pt]
The shapes are not strictly triangles and circles for scientific purposes. The image is closer to lifestyle. Also, the quality (in terms of resolution) of the image is not what one would expect in modern science.
\end{tabular}\\

\end{tabularx}
\caption{\textbf{Scientificness Guideline Examples} \\ (Scores are averaged across multiple annotators)} 
\end{table*}

==> structure/introduction.tex <==
\section{Introduction}
% this could mean to write an introduction to conduct a scientific experiment or to help make a plot,the last use case is ours. and, to my knowledge, there is no knowledge on how good the latest models are for this use case .and we make a sort of structured taxonomy, or so, for this use case


% However, a key need remains underexplored: generating scientific visualization, i.e., illustrative figures, charts and plots. Scientific visualization is essential for conveying complex ideas, data, and concepts. From charts to intricate diagrams, these visuals are crucial tools for researchers, educators, and students. Automating the creation of accurate scientific images from text could greatly enhance scientific communication and production.


Artificial intelligence (AI) has become an increasingly valuable tool in academic research, offering support across various aspects of the scientific process~\citep{elicit2024, chen-eger-2023-transformers, lu2024ai, info15060328, shao2024assistingwritingwikipedialikearticles}. For instance, platforms such as Elicit~\citep{elicit2024}\footnote{https://elicit.com/} and ResearchRabbit\footnote{https://www.researchrabbit.ai/} facilitate finding relevant literature for specific research topics. Tools like Grammarly assist with grammatical refinement and phraseology in academic writing and LLM assisted text production is nowadays common \citep{liang2024mapping}.  %and also explored in diverse scientific papers \citep{chen-eger-2023-transformers}. 
LLMs can also generate new ideas for scientific papers that rival the ideas produced by human scientists \citep{si2024llmsgeneratenovelresearch}. 
Even more holistically, approaches like The AI Scientist~\citep{lu2024ai} have demonstrated the capability to generate entire research output, %papers,
encompassing everything from initial conceptualization to experimental design and paper drafting.

Despite these advancements, a critical subproblem remains relatively unexplored: the AI-driven generation of scientific visualizations, including illustrative figures, charts, and plots \citep{voigt-etal-2024-plots}. These visual elements play a pivotal role in scientific communication \citep{Lee2016ViziometricsAV}, serving as essential tools for researchers, educators, and students to convey complex ideas, data, and concepts. The ability to automate the creation of accurate scientific images from textual descriptions could significantly enhance both the efficiency and effectiveness of scientific communication and production. Compared to previous attempts at automating image generation, AI-driven generation of scientific visualizations does not strictly rely on tabular data input~\citep{DBLP:conf/medes/YamadaOT18}, does not require cumbersome parameter adjustments~\citep{inproceedings_scipy}, and produces a variety of outputs beyond just statistical images~\citep{article_seaborn}. 
%The AI-driven approach %offers 
%promises 
%greater flexibility and power.


Scientific visualizations often require precise spatial composition, accurate numeric representations, and correct attribution of complex scientific objects. These elements must %often 
be combined in ways that adhere to established conventions within scientific domains. While general-purpose text-to-image models have made significant strides~\citep{esser2024scalingrectifiedflowtransformers, touvron2023llamaopenefficientfoundation, ramesh2021zeroshottexttoimagegeneration}, the requirements, e.g., precise and high-resolution graphical representations, %understanding abstract concepts over text, 
pose unique challenges for scientific image generation, as %shown 
illustrated in Figure~\ref{fig:teaser_intro}. Moreover, the representation of objects in scientific domains—such as batteries in circuit diagrams or %binary 
trees in graph theory—differs significantly from their appearance in real-life images. 
%Researchers have observed a decline in performance when generated images contain complex layouts or multiple objects. This issue poses significant challenges for scientific image generations~\citep{foong2023challengesimagegenerationmodels, gani2024llmblueprintenablingtexttoimage}.



% The rapid progress of multimodal large language models (LLMs) has transformed AI, enabling the generation of high-quality images from text. These models excel in creating visuals across diverse domains, from art to photorealism. 


%Current evaluations of text-to-image models primarily focus on general image quality, aesthetic appeal, and text-image alignment for everyday scenes. However, these metrics fall short when assessing the specific requirements of scientific visualization. The lack of a comprehensive benchmark tailored to scientific image generation has hindered our understanding of how well existing models perform in this crucial domain.
%-------------



In response to this need, we present \ourmodel{}, a comprehensive benchmark aimed at evaluating the capabilities of multimodal LLMs in generating scientific images conditioned on textual descriptions. 
Our benchmark includes a diverse set of skills that test %the 
key dimensions of scientific image production 
individually and in combination, covering a wide range of scientific 
objects, their attributes, and relations. 
%We evaluate five state-of-the-art LLMs—--GPT4-o~\citep{}, Llama~\citep{}, AutomaTikZ~\citep{}, Dall-E~\citep{}, and StableDiffusion~\citep{}---using two modes of output generation: code-based outputs (Python, TikZ) and direct raster image generation. Additionally, we examine performance across four different input languages: English, German, Farsi, and Chinese.
As scientific figures are often generated with high-level coding languages such as TikZ or Python, we evaluate standard LLMs (all capable of generating code output) such as \llama{} and \gpt{4o}, in addition to inherent multimodal models such as \dalle{} on \ourmodel.  



\begin{figure}%{0.8\textwidth}
    \centering % Answer: [trim={left bottom right top},clip]
    \includegraphics[trim={0 8cm 0 0 },clip, width=0.75\textwidth]{latex/plots/SciPlot_teaser.pdf}
    \caption{Illustration of scientific text-to-image generation. The text shown below is the generation query. Images on the left meet the expectations for general text-to-image tasks, while those on the right highlight the specific requirements of scientific image generation. All figures are from our \ourmodel{} experiments.}
    \label{fig:teaser_intro}
\end{figure}


Our findings highlight the need for continued research in enhancing the capabilities of multimodal LLMs for scientific image generation. By providing a standardized benchmark and in-depth analysis, \ourmodel{}  aims to drive progress in this critical area, ultimately supporting more efficient scientific %communication and collaboration.
image production. 
%The evaluation, conducted with 11 expert annotators from mathematics and computer science backgrounds, reveals that while all models face challenges in this task, GPT4-o produces high-quality results for simpler prompts involving individual dimensions. However, significant gaps remain, particularly in tasks requiring combined reasoning across multiple dimensions.

Key contributions of this work include:
\begin{itemize}
\item We provide a benchmark, \ourmodel, for testing the model capability of scientific text-to-image generation along (predominantly) three understanding dimensions: numeric, spatial, and attribute comprehension.
%\item A diverse dataset of textual captions paired with desired reference images.
\item We explore five %\todo{SE: below 7. Should maybe use one number and explain it}
state-of-the-art models on \ourmodel{}, both code-based and genuine multimodal.\footnote{Counting models with different outputs as distinct, we explore up to 8 different models, \emph{viz.}, (1) \automatikz, (2) \llama{}, (3) \stablediffusion, (4) \dalle, (5) \gpt{4o}, where \llama{} and \gpt{4o} use both (6) TikZ and (7) Python as output. For our multilingual evaluation, we further include (8) the recent OpenAI-o1 with python output.}
\item We comprehensively assess the models using almost a dozen human scientists\footnote{Our scientists are PhD students and higher. We use the term `scientist' to differentiate them from crowd-workers or early career academics such as Bachelor students.} 
across three evaluation aspects: correctness, relevance, and scientificness, and four languages: English, German, Chinese, and Farsi.
\item We analyze model performances across different object types, comprehension dimensions, and input languages.
\item We provide human evaluation scores for $\sim$3k generated scientific images, totaling an annotation value of approximately 3,000 USD.\footnote{For English, we evaluate 404 prompts for 7 different models, yielding 2828 individual images (308 of which have compile errors, receiving an automatic score of zero). For the later multilingual phase, we evaluate 460 images (58 with compile errors). In total, we thus evaluate 3288 prompts, 366 of which have compile errors.} 
These evaluation scores serve as a ``ground truth'' for the evaluation of generation performance and support future research on developing automated metrics for assessing scientific images.
\end{itemize}



\begin{comment}
    

\todo[inline]{----}
Multimodal large language models (LLMs) have exhibited impressive proficiency in generating high-quality images from textual descriptions~\citep{}. Despite these advancements, their effectiveness in generating scientific images has received relatively little attention. The generation of scientific images poses distinct challenges, as it necessitates precise spatial composition, accurate numeric representation, and correct %attribute binding, 
attribution of complex scientific objects, 
often in combination~\citep{}. 
Mastery of these abilities  --- which are also difficult for both experienced and aspiring human researchers --- is crucial for creating visual representations that accurately convey intricate scientific concepts and data. Models that can assist in this endeavor might provide tremendous support for human scientists, facilitating, accelerating and further automatizing scientific text production \citep{lu2024aiscientistfullyautomated}.
\end{comment}



==> structure/methods_orig.tex <==



\section{\ourmodel}

% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[width=.85\textwidth]{checking_list_new.pdf}
%     \caption{Taxonomy for designing generation queries.}
%     \label{fig:checking_list}
% \end{figure*}

\subsection{Task Setup}\label{sec:method_task_setup}
he 
\ourmodel{} %task 
evaluates the capability of multimodal LLMs to generate scientific graphs from textual descriptions. 
We design prompts that require models to understand and visualize scientific concepts, emphasizing three key dimensions of understanding:
%
(a) \textbf{Spatial understanding}: Assessing the models' ability to interpret and represent spatial relationships between objects, such as ``left of'' and ``on top of''.
(b) \textbf{Numeric understanding}: Evaluating the models' capacity to handle and visualize numerical requests accurately, such as the exact number of objects or requests like `more' and `half'.\footnote{The articles `a' and `an' are not interpreted as numerical descriptors.}
(c) \textbf{Attribute binding}: Testing the models' ability to correctly represent object attributes such as color, size, and shape.
Figure~\ref{fig:understanding_examples} demonstrates these three key dimensions of understanding. 

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=.7\textwidth]{latex/plots/understanding_dimension.pdf}
    \caption{Illustration of the three understanding dimensions. The first row shows the individual dimensions of Attribute, Numeric and Spatial understanding. The second row illustrates the combination of two or three dimensions.}
    \label{fig:understanding_examples}
\end{figure*}


\paragraph{Output mode} The task involves generating images either (i) \textit{directly text-image} 
or (ii) \textit{text-code-image} through intermediate code (Python or TikZ) --- which then has to be compiled to images --- based on textual prompts. 



\paragraph{Prompting} We instruct the models to generate scientific graphs with prompts. Each prompt consists of an \emph{auxiliary instruction} and a \emph{generation query}. The auxiliary instruction is used to constrain the model to generate scientific graphs in either (i) direct text-image or (ii) text-code-image mode. 
Language models can exhibit sensitivity to variations in prompts \citep{Leiter2024PrExMeLS}. 
%For example, %seemingly semantic-similar 
%\senew{highly similar} 
%prompts such as `Generate a scientific figure using Python code, strictly following the description below' and 'Please use Python code to generate a scientific figure' \senew{might} yield divergent outputs. 
To mitigate the impact of this variability and ensure a fair comparison between models, we conduct %systematic preliminary 
pilot tests to find prompts that generally lead all tested models to generate required output type (i.e., Python code, TikZ code, or images) in a scientific style. Our resulting auxiliary instructions are 
shown in Table \ref{table:base_instructions} in \cref{generation_instruction}. %\todo{SE: this seems exaggerated - we only made small-scale tests, did we? I think we should do at least one more large-scale exploration}
%We leave the systematic research of prompt sensitivity of models to future work. 
%The generated 
 Examples of code and image output are presented in \cref{code_output} and \cref{appendix_output_example}. 




\subsection{Dataset Construction}\label{sec:dataset_construction}


We begin with a comprehensive survey of relevant scientific datasets and benchmarks, as detailed in~\cref{tab:evaluation_dataset_summary} in~\cref{app:benchmark_survey}, also including math and science textbooks. This gave us the intuition that scientific graphs are described by objects and their properties (attributes) as well as their relative positioning (spatial relations) and numeric information (e.g., how many objects). Additionally, annotations often emphasize parts of the scientific image. 
\iffalse
To initially assess model performance, \todo{SE: so, we already use models to construct the data?}
we randomly sampled textual descriptions associated with scientific graphs from these datasets.\footnote{We excluded entries requiring non-textual inputs.}
Through preliminary experiments, we observed that current state-of-the-art models, including commercial systems, struggle with these textual descriptions in both text-to-image and text-code-image generation tasks. While some datasets, such as ArXivCap~\cite{li2024multimodal} and SciBench~\cite{wangscibench}, could theoretically be adapted for text-to-image evaluation by using figure captions or textual descriptions as inputs and the corresponding scientific figures as ground truth, we identified two major limitations: (1) the captions or descriptions often lack the comprehensive information needed for accurate figure reproduction, and (2) the generation complexity of these figures exceeds the current capabilities of state-of-the-art models. %Therefore, we develop a specialized dataset to evaluate the scientific visualization capabilities of Large Language Models (LLMs) and Multimodal LLMs.
\todo{SE: I don't like this paragraph. If there's something else we could have used, then we probably should have used it? But I think our goal is not to test out arbitrary captions --- we could have used Datikz for this --- but specificially see what's going wrong where. I suggest to remove this whole paragraph or reduce it to 1.5 sentences.}
\fi 

Thus, we develop prompt requirements to ensure that varying aspects of scientific text generation are covered. We require that each prompt must explicitly define: 
(a) the core visual elements (objects) to be generated in the graph, e.g.\ cycle, square, etc.; (b) specific attributes of the object (\textbf{attribute binding}), e.g., red cycle, or count of the object (\textbf{numeric}), e.g.\ three cycles. 
the positioning arrangement and placement (\textbf{spatial}) of objects within the graph, e.g.\ on the bottom or in relation to another object (to the left). %Fourthly and optionally, 
(d) We finally consider 
any required labels, legends, or additional textual elements (annotations). %\todo{SE: then we have to include this in our earlier announcements?}
Further, for graphs containing multiple objects, the prompt must additionally specify the quantity of each object type, the relative spatial or logical relationships between objects, and the individual properties of each object group. Individual aspects are typically optional, i.e., not every prompt has to specify numerical or spatial components. Specific details on dataset construction follow below.

\paragraph{Generation Queries $Q$} 
We adopt a structured methodology that leverages a \textbf{dictionary $D$} along with a set of \textbf{query templates $T$} to create a diverse, comprehensive, and traceable set of generation queries $Q$ for the \ourmodel{} evaluation dataset. 


\input{latex/structure/table-example_copy}



\textbf{Dictionary $D$} defines key elements relevant to scientific figures, including objects (e.g., square and circle), attributes (e.g., color and size), spatial relations (e.g., left, right, between), and numeric values (e.g., three, five, two more). To construct this dictionary, we begin by building the list of objects. First, we manually extract %the 
frequent object entities from \textsc{Datikz}~\citep{belouadi2024automatikz}, an image-caption dataset derived from scientific publications.

\footnote{\textsc{Datikz} is unsuitable for our exploration, as it contains textual descriptions `in the wild' and additionally its captions are often unsuitable for reconstructing the output image at hand.} We filter out objects highly dependent on the context of the original paper, such as mathematical formulas adjacent to figures and line segments with specific values. Additionally, we simplify complex objects—such as intricate circuit designs and automata intended for specific applications. %, yielding a %final set of 45 objects. \todo{SE: can that be listed in the appendix?}
Next, we manually define representative spatial relations, such as ``to the left'' and ``at the center of'', to describe the positions of objects within graphs. Additionally, we create attribute sets to capture detailed object properties, including size, color, and line thickness. Numerical requests are also incorporated into the dictionary to replace values in bar charts or assess models' accuracy in representing object counts. We then collect attributes and relations that appear at least three times and then manually compile a list of attributes and spatial relations by merging similar ones and removing %ones that are 
domain-specific ones.
%}% \todo{SE: What? Compile A based on A?}
% To ensure reliability and representativeness, we retain only those attributes and relations that appear at least three times.% Specifically, we extract object entities from \textsc{Datikz}~\cite{belouadi2024automatikz} and filter the top 20 most frequent ones. We further manually filter out rare or challenging objects, such as xxx and xx, and end up with xxx objects. We further extract the descriptions associated with these objects from \textsc{Datikz}, and collect all appeared attributes and relations. We filter out the attributes and relations that appear less than three times. 

At the top level, $D$ is organized into classes for objects, attributes, numeric, and spatial relationships. Each class then contains a list of descriptive words specifying the class.
When selecting a descriptive word from $D$ for a given blank in the query templates $t_i$, we first locate the specific list corresponding to the word class and then randomly choose an item from it.\footnote{During the word collection process, we excluded complex and rare terminologies due to potential bias. Consequently, attributes such as `hinges' and `hyperstatic structures' were omitted.} For clarity, we present a snippet of $D$ below:
{\small
\begin{verbatim}
D = {"2D_objects": ["square", "circle", ...],
     "3D_objects": ["cube", "sphere", ...],
     "colors": ["red", "blue", ...],
     "spatial_relations": ["left", "right", ...],
     ...}
\end{verbatim}
}
We define a set of \textbf{query templates $T$}, where each template $t_i \in T$ is one or several sentences %or several sentences.
with one or more placeholders. These placeholders are designed to be filled with elements $d_j \in D$, which may include objects, attributes, or relations. To construct a generation query $q_k \in Q$, we select a query template $t_i$ and populate its placeholders with appropriate attributions from $D$. This process allows us to create diverse queries with meta-info. %We have 101 templates in total.
The final step in preparing our generation prompt involves prefixing the constructed generation query $q_k$ with task-specific auxiliary instructions, as detailed in Section~\ref{sec:method_task_setup}. This structured approach ensures transparency and flexibility across diverse queries, while minimizing potential biases toward specific objects, attributes, and other contextual elements.



% \begin{table*}[th!]
%     \centering
%     \small
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|l|l|l}
% \hline
% \multicolumn{1}{c|}{\textbf{Object Type}} & \multicolumn{1}{c|}{\textbf{Query Template}} & \multicolumn{1}{c|}{\textbf{Dictionary Value}} & \multicolumn{1}{c}{\textbf{Generation Query}} \\ \hline
% 2D shape & \begin{tabular}[c]{@{}l@{}}Some \{object-plural\} of different\\ sizes.\end{tabular} & ellipses & Some ellipses of different sizes. \\ \hline
% 3D shape & \begin{tabular}[c]{@{}l@{}}Two \{color\} spaces divide a/an \\ \{3D-object\} into four parts.\end{tabular} & blue, pyramid & \begin{tabular}[c]{@{}l@{}}Two blue spaces divide a \\ pyramid into four parts.\end{tabular} \\ \hline
% Chart & \begin{tabular}[c]{@{}l@{}}In a bar chart, a/an \{color-1\} bar is \\ to the right of a/an \{color-2\} bar, \\ and the leftmost bar is the \{tallest/\\ shortest\} in the chart.\end{tabular} & blue,orange, tallest                      & \begin{tabular}[c]{@{}l@{}}In a bar chart, a blue bar is \\ to the right of an orange bar, \\ and the leftmost bar is the \\ tallest in the chart.\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Graph theory \\ (Node \& Edges)\end{tabular} & \begin{tabular}[c]{@{}l@{}}A binary tree with a total of \\ \{number\} nodes.\end{tabular} & 12 & \begin{tabular}[c]{@{}l@{}}A binary tree with a total \\ of 12 nodes.\end{tabular} \\ \hline
% Matrix                                                                  & \begin{tabular}[c]{@{}l@{}}A \{number\_1\}-by-\{number\_2\} \\ matrix.\end{tabular} & six, three & A six-by-three matrix. \\ \hline
% Real-life object                                                        & \begin{tabular}[c]{@{}l@{}}There are \{number-1\} boxes on \\ a \{number-2\} degree slope.\end{tabular}                                                                                       & 4, 30                                     & \begin{tabular}[c]{@{}l@{}}There are 4 boxes on a 30\\ degree slope.\end{tabular} \\ \hline
% Table & \begin{tabular}[c]{@{}l@{}}A table with \{number-1\} rows and\\ \{number-2\} columns. The row \\ index is marked in the first column.\end{tabular} & three, five & \begin{tabular}[c]{@{}l@{}}A table with three rows and\\ five columns. The row index\\ is marked in the first column.\end{tabular} \\ \hline
% Annotation & \begin{tabular}[c]{@{}l@{}}The English text (the name of the \\ object) is \{preposition\} the \\ \{object\}.\end{tabular} & to the left of, triangle                  & \begin{tabular}[c]{@{}l@{}}The English text (the name of\\the object) is to the left \\ of the triangle.\end{tabular} \\ \hline
% Function \& Coordinate & y = \{function\} and its inverse function. & 3\textasciicircum{}\{x\} & y = 3\textasciicircum{}\{x\} and its inverse function.                                                                                                          \\ \hline
% \end{tabular}}
%     \caption{Illustration of constructing generation queries.}
%     \label{tab:prompt_template}
% \end{table*}




%Our dataset 
Further, \ourmodel{} is crafted to cover a wide range of scientific graph types and complexities. We classify the object types 
% \todo{SE: so what is more complex; function or 2D geometric change? I don't think we have any order of complexities. \\Leixin: different models perform differently regarding the obejct challenges, should we take the average across all models? and add it here? SE: I am not sure but complexity seems to suggest that something is more complex than something else. Is that true? (3D more complex than 2D, etc.?  Leixin yes, other than this point, it's hard to assume sth, we can assume those without a library can be harder,like real-life-object modeling). SE: right, but then I would not use the term complexity at all.}
of all prompts based on the following categories: 2D geometric shapes, 3D geometric shapes, charts, graph theory representations, matrices, real-life object modeling, tables, additional annotations, functions \&  coordinates. For each category, we create multiple templates that vary in complexity and combine different aspects of spatial, numeric, and attribute understanding. For each template, we create four different generation queries by sampling different elements from the dictionary $D$. In total, we have 101 query templates and 404 generation queries. Examples of \ourmodel{} are shown in Table \ref{tab:prompt_template}. 
%\todo{SE: how do we classify `with a border'? What is `divide into N parts'? Spatial? What is `function x and its inverse function'?}




\subsection{Evaluation}
We employ a multi-faceted evaluation approach to assess the quality and accuracy of the generated scientific graphs:


\begin{wraptable}{l}{0.5\linewidth}
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{rccc}
\hline
\textbf{Agreement} & {\color[HTML]{333333} \textbf{Correctness}} & {\color[HTML]{333333} \textbf{Relevance}} & {\color[HTML]{333333} \textbf{\begin{tabular}[c]{@{}c@{}}Scientificness \end{tabular}}} \\ \hline
Joint Spearman $r$   & {\color[HTML]{333333} 0.67}                 & {\color[HTML]{333333} 0.62}               & {\color[HTML]{333333} 0.73}                                                                \\
Joint Pearson $r$    & 0.70                                        & 0.64                                      & 0.71                                                                                       \\

Joint Weighted Kappa       & 0.50 & 0.41 & 0.45 \\ \hline

Pair Spearman $r$ (Eng)   & {\color[HTML]{333333} 0.73}                 & {\color[HTML]{333333} 0.64}               & {\color[HTML]{333333} 0.63}                                                                \\
Pair Pearson $r$  (Eng)   & {\color[HTML]{333333} 0.75}                 & {\color[HTML]{333333} 0.65}               & {\color[HTML]{333333} 0.63} \\ 
Pair Weighted Kappa (Eng)         & 0.61 & 0.52 & 0.47 \\ \hline

Pair Spearman $r$ (Multi)        & 0.80 & 0.75 & 0.73 \\
Pair Pearson $r$ (Multi)         & 0.80 & 0.77 & 0.79 \\
Pair Weighted Kappa (Multi)       & 0.64 & 0.60 & 0.66 \\ \hline

Pair Spearman $r$ (Eng + Multi)  & 0.76 & 0.68 & 0.67 \\
Pair Pearson $r$ (Eng + Multi)   & 0.77 & 0.69 & 0.67 \\
Pair Weighted Kappa (Eng + Multi) & 0.62 & 0.55 & 0.52 \\

\hline
\end{tabular}
}
\caption{Agreement of joint evaluation in the calibration session (joint) and pair agreement (agreement across all examples of two sets of annotations) in the final evaluation for English and multilingually.}
\vspace{0pt}
\label{tab:agreement}
\end{wraptable}

\paragraph{Human Evaluation} %We engage 11 scientists (7 early and advanced PhD students, 2 PostDocs and 2 faculty members) to 
Our human evaluators assess the generated images based on three criteria: \textbf{Correctness}: Assessing the accuracy of the visual representation in relation to the textual prompt.
\textbf{Relevance}: Evaluating how well the model avoids generating redundant or irrelevant objects or attributes of objects. 
\textbf{Scientific Style}: Evaluating the appropriateness of the image for use in scientific publications.
Each criterion is rated on a scale from 1 to 5, with 5 being the highest score. An additional score of 0 is assigned in cases where code generation cannot be compiled into an image due to compilation errors.\senew{\footnote{While assigning a score of 0 may seem harsh, we also report results when ignoring all compile errors, which would constitute an upper bound.}} 
The detailed evaluation guideline is given in \cref{app:evaluation_guideline}.

% While correctness measures whether the output correctly represents the input, relevance indicates whether no additional objects or relations are present in the output image. Note that we do not assess the intermediately generated code by itself.


%On top of evaluation the three aspects above, we further examine the following aspects: 

% Besides this human annotation, we also measure the 
% \textbf{Compile Error Rate}: For models that generate code (Python or TikZ), we track the rate of compile errors to assess the reliability of the code generation process.


% \todo{SE: I think this below is part of the analysis, i.e., object complexity analysis, not part of the human annotation}
%\textbf{Object Complexity Analysis}: We analyze model performance across different object types to identify strengths and weaknesses in handling various scientific graph categories.
%\textbf{Reasoning Ability Assessment}: We evaluate the models' performance on tasks requiring spatial reasoning, numerical reasoning, attribute binding, and combinations thereof.
%\textbf{Model Stability}: We assess the consistency of each model's performance by calculating the standard deviation of scores for multiple examples generated from the same template.


% \todo{SE: besides `delve into', `ensure' seems to be the new LLM indicator, isn't it? :-), CASS: haha TRUE}







We employ a panel of 11 expert annotators, carefully selected to represent the target users of scientific plots and graphs. This panel consists of: eight Ph.D. students, one postdoctoral researcher, 
and two faculty members from mathematics and computer science, ensuring domain expertise in evaluating scientific visualizations. We provide each annotator with detailed annotation guidelines given in the Appendix~\ref{app:evaluation_guideline}. 
Furthermore, before formal annotation distribution, we conduct a \textbf{calibration session} to match the understanding of the annotation standard. We randomly assign examples to annotators and further assign at least two annotators per instance to mitigate annotation biases. 


\paragraph{Agreements} \cref{tab:agreement} presents the agreement scores (Spearman's $r$, Pearson's $r$ and weighted Kappa) from both the small-scale calibration session (joint evaluation: 315 images are evaluated by all evaluators) and the later pairwise evaluation (pair evaluation: every image is evaluated by a pair of evaluators) using various models (see Section~\ref{sec:evaluation_results}).
% Pair agreement is obtained by comparing two sets of annotations across all examples. 
A relatively strong positive correlation with Pearson $r$ and Spearman $r$ between 0.62 and 0.80 is observed across all evaluation criteria. %In the final evaluation phase, the correctness dimension exhibits the highest correlation, indicating the reliability of human assessments in evaluating the alignment between the prompt and the generated output. 
Weighted kappa, a chance-corrected measure of agreement for ordinally scaled samples, is within commonly accepted ranges for agreement, with almost all
measures above 0.5. The multilingual evaluation, conducted by a subset of 6 more experienced evaluators, shows a higher level of agreement than the English evaluation. Overall, weighted kappa is 0.62 for correctness for combined English and multilingual evaluation and above 0.52 for relevance and scientificness.

We tax the value of our evaluation at roughly 3,000 USD, with up to 11 annotators involved for up to 7 hours each, all working for a conservative estimate of 40 USD per hour (including taxes), on average.


\paragraph{Automatic Evaluation} We also test how well recent automatic text-to-image evaluation metrics correlate
with our human judgements. We explore 5 recent multimodal metrics. These achieve a highest Kendall correlation with human scores of 0.26, where the agreement on the correctness dimension is highest and lowest on scientificness (maximum Kendall of 0.15). This underscores the value and necessity of our human annotation campaign. Details are given in \cref{app:autometrics}.


% \senew{Weighted kappa, an agreement measure of ordinally scaled samples, is acceptable according to commonly accepted ranges for kappa. It is highest for correctness and lowest for scientificness, but all are above 0.5. 
% Multilingual Evaluation has higher agreement than that of English because the evaluators of multilingual generation received more training and an additional round of calibration phase.}


% Pearson and Spearman are about 0.15 points higher. Multi-eval has higher scores because annotators are better calibrated} \todo{SE: fix this sentence please}

%\todo{SE: we need to explain a lot here--- e.g. (1) what is joint, (2) what is paired, (3) weighted kappa, (4) the panel size difference between English and multi, (5) multi, (6) what is weighted kappa. Note that parts of the results can go to the appendix}



%To ensure reliability and consistency in the evaluation process, we implement the following measures:
%\begin{itemize}
%    \item Inter-rater Agreement: We calculate Krippendorff's alpha to assess the agreement between annotators. This metric is chosen for its ability to handle multiple raters and ordinal data.
%    \item Calibration Sessions: Prior to the main evaluation, we conduct calibration sessions where annotators discuss and align their understanding of the evaluation criteria using a subset of diverse examples.
%    \item Randomized Assignment: Images are randomly assigned to annotators to mitigate potential biases.
%    \item Cross-validation: All annotators evaluate a subset of images (20\%) to allow for cross-validation of ratings.
%    \item Qualitative Feedback: Annotators are encouraged to provide brief qualitative feedback, especially for edge cases or particularly noteworthy examples.
%\end{itemize}


%We aim to present a comprehensive human evaluation approach that not only provides quantitative metrics to assess model performance, but also offers valuable qualitative insights into the strengths and limitations of current scientific graph generation capabilities. The involvement of domain experts ensures that our evaluation captures nuanced aspects of scientific visualization that may be missed by automated metrics alone.

%The results from this human evaluation are then analyzed in conjunction with other metrics such as compile error rates and model stability to provide a holistic assessment of the models' capabilities in scientific graph generation.



==> structure/related.tex <==
\section{Related work}\label{sec:related}


% Some recent related work:
% \begin{itemize}
%     \item \url{https://arxiv.org/abs/2407.10972}
% \item \url{https://chartmimic.github.io/}
% \item \url{https://aclanthology.org/2024.lrec-main.1119.pdf}
% \item Benchmarks for multimodal failures (reasoning, spatial understanding, etc.?
% \end{itemize}


% In computer vision and multimodal studies, there are benchmarks and datasets serving for various purposes, including object detection, e.g. MS COCO 
% \cite{lin2014microsoft}, image classification, such as CIFAR-10, CIFAR-100 \cite{krizhevsky2009learning} and ImageNet \cite{5206848}, hand-written digits recognition: MNIST \cite{6296535}, and image captioning (\citealp{sharma-etal-2018-conceptual} and Microsoft COCO Captions by \citealp{chen2015microsoft}). In the scientific domain, Paper2Fig100k \cite{rodriguez2023ocr} contains over 100k images of figures and texts extracted from research papers.

% \end{comment}

% In computer vision and multimodal studies, benchmarks or datasets serving various purposes, including object detection (MS COCO, 
% \citealp{lin2014microsoft}), image classification (CIFAR-10, CIFAR-100, \citealp{krizhevsky2009learning} and ImageNet \citealp{5206848}), hand-written digits recognition (MNIST, \citealp{6296535}), image captioning (\citealp{sharma-etal-2018-conceptual} and Microsoft COCO Captions \citealp{chen2015microsoft}). 
In computer vision and multimodal studies, there are many benchmarks and datasets serving %for 
various purposes, including object detection %\citep{lin2014microsoft} 
(\citealp{lin2014microsoft}), image classification (\citealp{krizhevsky2009learning}, \citealp{5206848}), hand-written digits recognition (\citealp{6296535}), and image captioning (\citealp{sharma-etal-2018-conceptual}, \citealp{chen2015microsoft}), but the majority focus on real world images. 
Although datasets like Paper2Fig \citep{rodriguez2023ocr} and DaTikZ \citep{belouadi2024automatikz,belouadi2024detikzifysynthesizinggraphicsprograms} include scientific figures and captions extracted from research papers, %a comprehensive evaluation of models' reasoning capabilities in the scientific domain remains lacking. 
there is no structured evaluation of the limitations and capabilities of scientific text-to-image models. 
In Section \ref{image-input} and \ref{image-generation}, %the following two subsections, 
we review existing benchmarks designed to assess model abilities: visual understanding (e.g., using images as inputs \citep{thrush2022winoground, huang2023t2i, wuevaluating}, discussed in \cref{image-input}) and ability of text-to-image generation (\cref{image-generation}). All surveyed datasets and benchmarks in this study are summarized in \cref{tab:evaluation_dataset_summary} in \cref{app:benchmark_survey}. 

% \todo[inline]{SE: I would remove most mentions to reasoning. Do you simply mean: 4.1 is about benchmarks for understanding images and 4.2 is about benchmarks for generating images? Leixin: yes, but 2.1 and 2.2 not 4.1 and 4.2}

% We also highlight the advantages of our dataset in evaluating these capabilities across multiple dimensions.


% \subsection{Benchmarks for Reasoning}


% Recent benchmarks (\citealp{thrush2022winoground}, \citealp{huang2023t2i}, \citealp{wuevaluating}) focus on more challenging aspects of model performance, particularly in areas such as visual reasoning (e.g., using images as inputs, as discussed in \cref{image-input}) and reasoning in text-to-image generation (\cref{image-generation}). These benchmarks test models' ability to understand and reason about complex concepts, including spatial, temporal, and logical relationships, and to generate corresponding images as outputs.


\subsection{Image as Input}\label{image-input}
Benchmarks that use images as input often take the form of visual question answering (VQA), where images are paired with questions about their content \citep{biten2019scene,das2024exams,yue2023mmmu,wangscibench}. For example, the Multimodal Visual Patterns (MMVP) Benchmark \citep{tong2024eyes} focuses on challenging cases, comprising 150 CLIP-blind pairs (images that the CLIP model perceives as similar despite clear visual distinctions) with questions designed to probe specific image details, such as relative position, object counting, or other attributes.

In the scientific domain, VQA examples are typically sourced from exams, quizzes, or textbooks \citep{yue2023mmmu,lu2024mathvista,li2024multimodal}. Additionally, ScienceQA \citep{lu2022learn} is a benchmark that uses images as contextual inputs for questions, rather than directly asking about the image's content. This dataset also incorporates Chain of Thought (CoT) reasoning to enhance interpretability alongside the answers. CharXiv \citep{wang2024charxiv} evaluates models' abilities to describe and reason about charts through multiple-choice questions.

Another type of visual understanding benchmark focuses on caption-image alignment. Winoground \citep{thrush2022winoground}, for instance, challenges models to match images with their corresponding captions. The dataset includes pairs where objects or predicates are swapped, such as ``there is a mug in some grass'' versus ``there is some grass in a mug'', to test fine-grained comprehension of texts. MMSCI \citep{li2024mmsci} extends this focus to the scientific domain, offering a figure-captioning benchmark spanning 72 subjects. Additionally, SciFIBench \citep{roberts2024scifibench} evaluates figure-caption alignment through tasks such as selecting the appropriate figure for a given caption or choosing the correct caption for a specific figure from multiple choices.


\subsection{Image as Output} \label{image-generation}
Compared to visual understanding, benchmarks that assess %the 
individual dimensions of %models' 
abilities in text-to-image generation models remain relatively %underexplored. 
scarce. 
One benchmark designed for this purpose is T2I-CompBench \citep{huang2023t2i}, which includes 6k compositional text prompts, categorized into three groups: attribute binding (e.g., color and shape), object relationships (e.g., spatial arrangements), and complex compositions. 
%However, a benchmark for evaluating the various reasoning abilities in scientific graph generation is currently lacking.
While we are inspired by this benchmark, we note that it does not target the scientific domain. 

In the context of vector graph and scientific figure generation, \cite{zou2024vgbench} develop %ed 
an evaluation set to assess models' abilities in prompt comprehension and vector graph generation. \cite{belouadi2024automatikz} introduce %d 
a dataset that pairs scientific paper captions (as input) with TikZ code (as output), which can be compiled into vector graphs. Additionally, \cite{shi2024chartmimic} explore %d 
models' capabilities to replicate chart images by converting them into Python code. %In contrast to these evaluation datasets, we designed \ourmodel{} with a more fine-grained approach, emphasizing key dimensions that are crucial for the scientific domain, but challenging for current models, such as scientific object representation, numerical reasoning, and spatial understanding.
Compared to these works, which focus on specific evaluation settings (such as TikZ or vector graphic %generation 
or chart generation), our evaluation setup is broader, %more nuanced, 
more targeted and more structured: we assess model performance across different input languages and output formats (TikZ vs.\ Python vs.\ plain image), object types and aspects of understanding. 



% However the benchmark for real-life image evaluation cannot evaluate the generation quality of scientific graphs. We highlight the distinctions between scientific graphs and general graphs and assume that scientific graphs should prioritize accuracy in representing scientific concepts and ideas. This includes ensuring the accuracy of numerical values and adhering to certain conventions when simplifying real-life objects into graphical representations (e.g., representing a "battery" with a rectangle in a circuit diagram) in scientific books or papers.



% Although image-text alignment for general images can be evaluated with metrics like the CLIP score \cite{hessel2021clipscore}, such evaluations have not yet been extended to the scientific domain. In the scientific context, accuracy in both image generation and text description is paramount. It remains uncertain whether nuances such as the precision of numerical representations or the proportions of bars in a bar chart can be adequately captured by existing evaluation metrics.


 % the evaluation of image output is not as straightforward as the evaluation of the output or the answer of a question like dataset in \cref{image-input}.

% Moreover, evaluating scientific graphs poses challenges even for human evaluators, as it requires specialized scientific or professional knowledge. Crowd evaluation may be difficult due to the complexity of the scientific concepts involved. Even when captions and images are provided, human evaluators may struggle to assess the quality of scientific images if the information is presented in an uncontrolled manner.
% To address these challenges, we propose a novel approach.



\subsection{Evaluation of Text-to-Image Models}\label{sec:eval}

Existing evaluations of text-to-image models primarily focus on text-image alignment and image quality for real-world images, as demonstrated by benchmarks such as MS COCO~\citep{lin2014microsoft} and studies in \citet{sharma-etal-2018-conceptual} and \citet{chen2015microsoft}. Later works, such as \citet{lee2024holistic} and \citet{cho2023dall}, broaden the scope of evaluation to include aspects like aesthetics, originality, social bias, and efficiency, but these %assessments 
still remain within the domain of real-world images.

Benchmarks designed for evaluating real-life images are insufficient for assessing the quality of generated scientific graphs. Compared to general images, scientific graphs must prioritize accuracy in representing scientific concepts and ideas. This includes ensuring the precision of numerical values in charts or plots, and adhering to established conventions when translating real-world objects into graphical representations (e.g., depicting a ``battery'' in electric circuit diagrams within the domains of engineering and physics).%\todo[inline]{SE: what does simplifying mean here? And what's special about the battery thing? (also occurred in the intro, but I didn't get it)}


For figures in the scientific domain, metrics like CLIPScore and Fréchet Inception Distance (FID) are employed to assess the quality of generated graphics \citep{zou2024vgbench}. Additionally, \citet{shi2024chartmimic} utilize GPT-4V for automated evaluations of image quality. However, as highlighted by the MMVP benchmark \citep{tong2024eyes}, automated evaluations can be unreliable, particularly when recognizing precise directions in text and images, such as ``up'' and ``down''. The precision required for evaluating scientific graphs presents significant challenges for current automated metrics. To address this gap, we %develop a new evaluation benchmark with input from 11 scientists, offering a reliable assessment of model performance in the scientific domain.
resort to human evaluation instead of automatic evaluation, using a panel of 11 scientists. Additionally, we show that, indeed, standard multimodal metrics employed in the community have low correlations to our human annotators in our scientific domain.

% \todo[inline]{SE: I think the two most closely related works are these: (i) https://chartmimic.github.io/, (ii) https://arxiv.org/abs/2407.10972, (iii). Do we adequately discuss them and how are we different from them? Yes, I explained with two paragraphs, they are automatically evaluation}

% A few works have been done focusing on applications in domains of art, design, and medical imaging [13, 14].



% \subsection{Scientific Graph Generation}





% \todo[inline]{maybe merge it to the last section. Further, please adding citations.}




% \subsection{Evaluation of Scientific Image Generation}


% General benchmarks or metrics used to evaluate image generation may not necessarily be applicable to the scientific graph domain. We highlight the distinctions between scientific graphs and general graphs and assume that scientific graphs should prioritize accuracy in representing scientific concepts and ideas. This includes ensuring the accuracy of numerical values and adhering to certain conventions when simplifying real-life objects into graphical representations (e.g., representing a "battery" with a rectangle in a circuit diagram).


% Although image-text alignment for general objects can be evaluated using metrics like the CLIP score \cite{hessel2021clipscore}, such evaluations have not yet been extended to the scientific domain. In the scientific context, accuracy in both image generation and text description is paramount. It remains uncertain whether nuances such as the precision of numerical representations or the proportions of bars in a bar chart can be adequately captured by existing evaluation metrics.




% Moreover, evaluating scientific graphs poses challenges even for human evaluators, as it requires specialized scientific or professional knowledge. Crowd evaluation may be difficult due to the complexity of the scientific concepts involved. Even when captions and images are provided, human evaluators may struggle to assess the quality of scientific images if the information is presented in an uncontrolled manner.




==> structure/results.tex <==
\section{%Evaluation 
Experiments}\label{sec:evaluation_results}

We employ two types of models for image generation, corresponding to the two output modes described in Section~\ref{sec:method_task_setup}. For (i) direct text-%to-
image mode, we include \dalle{} and \stablediffusion{}; for (ii) text-code-image, we include \gpt4o{}, \llama{} and \automatikz{}~\citep{belouadi2024automatikz}, where the model is prompted to generate Python or TikZ code. %for generation query, we further compile the code to generate the plot or figure. 
\automatikz{} is %a model 
specifically %designed 
fine-tuned for generating TikZ code, therefore, we only prompt \automatikz{} to generate TikZ. 


\begin{wraptable}{l}{0.5\textwidth}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{rcccc}
\hline
\textbf{Model}   & \textbf{Correctness}        & \textbf{Relevance}          & \textbf{\begin{tabular}[c]{@{}c@{}}Scientific\\ style\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Compile\\ Error Rate\end{tabular}} \\ \hline
Automatikz       & 2.05 & 2.31 & 3.35                                                                & 0.04                                                                  \\
Llama\_tikz      & 1.78 & 1.94 & 2.61                                                                & 0.29                                                                  \\
GPT-4o\_tikz     & 3.50 & \textbf{3.67} & 3.75                                                                & 0.09                                                                  \\ \hline
Llama\_python    & 2.10 & 2.54 & 3.18                                                                & 0.28                                                                  \\
GPT-4o\_python   & \textbf{3.51} & 3.40 & \textbf{3.93}                                     & 0.07                                                                  \\ \hline
Stable Diffusion & 2.19 & 2.09 & 1.96                                                                & -                                                                  \\
DALL·E           & 2.16 & 2.00 & 1.55                                                                & -                                                                  \\ \hline
\end{tabular}
}
\caption{Overall model performance, averaged across instances (compile error of code output is penalized with score 0) and annotators. The column-wise highest is marked in bold.}
\label{tab:overall_performance}
\vspace{-20pt}
\end{wraptable}



% \begin{wrapfigure}{l}{0.5\textwidth}
%     \centering
%     \includegraphics[width=0.5\textwidth]{overall_e2206.pdf}
%     \caption{Overall Performance of Models.}
%     \label{fig:overall}
% \end{wrapfigure}

\textbf{Overall performance}: The overall model results are presented in \cref{tab:overall_performance}, showing averages based on per-instance human evaluations and further averaged across annotator pairs. Instances where code generation resulted in compilation errors are penalized with a score of 0. \footnote{A score of 0 does not apply if a compile error occurs due to missing TikZ code like $\backslash begin\{documentclass\}$. Models sometimes assume that a document has already been set up, so we check and add codes at head and tail for generated codes before compiling the image.} In \cref{appendix_results_without_0}, we show scores where compilation errors are ignored; potentially compilation errors could be fixed by self-consistency checks in future approaches. Overall, \textit{GPT-4o in text-code-image mode (GPT-4o\_tikz and GPT-4o\_python) stands out as the model achieving the best scores across all evaluation dimensions. However, %its average correctness score lies only between 3 and 4, indicating at least some mistakes on average in every image. More generally, 
it scores below 4 in all three evaluation dimensions, indicating at least some mistakes on average in every output.}
% Notably, no single model consistently outperforms others across these three dimensions. \todo[inline]{SE: well, our own text says that GPT4o outperforms all models across all 3 dimensions, right? Leixin: yes, the previous wording is a bit hard to understand. Another point I commented above:  if without_0, llama is the best for scientificness}


\textbf{Correctness}: \gpt{4o} outperforms all other models by a large margin (more than 1.3 points), achieving the highest scores for both the text-tikz-image (3.50) and text-python-image (3.51) output. All other models have correctness scores between 1.7 and 2.2, indicating low correspondence between instruction and output image. \llama{}\_tikz (1.78) and \automatikz{} (2.05) are the worst models. %It is interesting to observe that 
Interestingly, \llama{} performs considerably better with Python as output than with TikZ as output (2.10 vs.\ 1.78). Similarly, \gpt{4o} performs marginally better with Python as the coding language. 
When ignoring compile errors (Table \ref{tab:overall_result_without_0}), the code generation models become substantially better, especially \llama{} improves by almost 1 point, leaving the direct text-image  generation models \stablediffusion{} and \dalle{} among the worst models. 

% \todo[inline]{SE: Fig. 2 isn't cited Leixin: cited}

\textbf{Relevance}:  
%Similarly, \texttt{GPT-4o} also achieves the best performance in terms of relevance, particularly for images compiled from TikZ code (score\_relevance = 4.02), which is significantly higher than images compiled from \texttt{GPT-4o\_python} code (score\_relevance = 3.64), \texttt{Llama\_python} code (3.52), and \texttt{llama\_tikz} code (2.72). In this dimension, \texttt{Automatikz} (2.41) outperforms \texttt{Stable Diffusion} and \texttt{DALL·E}.
%\todo[inline]{Leixin: as we replaced the table with a including-0 version, now it's difficult to just change values in the  writing of this relevance paragraph}
\gpt{4o} also dominates relevance, but with a smaller margin (1.13 vis-a-vis the second best model \llama{} with Python output). \llama{} again prefers Python output while \gpt{4o} prefers TikZ. Visual models \stablediffusion{} and \dalle{} often include irrelevant details in their output and are among the worst; see \cref{tab:model_examples} in \cref{appendix_output_example} for examples. 




\textbf{Scientificness}: %Style Evaluation}
Images converted from Python or TikZ code receive notably higher scores ($>$ 2.5) in scientific style compared to direct image generation from \dalle{} and \stablediffusion{} %(score\_scientific\_style < 2.0). 
($<$ 2). 
This suggests that code output as an intermediate step offers a significant advantage for scientific graph generation, as opposed to visual models that are primarily trained on real-life images.

% \todo[inline]{SE: Table 5 needs bold ; all tables need bold}

However, a significant drawback of models that generate code is the potential for compilation failures. For instance, \gpt{4o} experiences 35 TikZ code and 27 Python code compilation errors. \llama{} has even much higher failure cases: 116 for TikZ mode and 113 for Python code, representing approximately 28\% of all prompts. \texttt{Automatikz} performs best in terms of compilation success, with only 17 cases in total. The low scores observed for \llama{} in \cref{tab:overall_performance} can largely be attributed to penalties for these compilation errors. %Performance results excluding penalization for compilation errors are presented in \cref{tab:overall_result_without_0} in %Appendix 
%\cref{appendix_results_without_0}.
If these were ignored (or could be fixed), \llama{} would outperform \automatikz{} as shown in \cref{tab:overall_result_without_0} in \cref{appendix_results_without_0} (note, however, that the comparison for both models includes different instances, thus is not fully fair in the table). %\todo{SE: potential critique - evaluate on the same set of compiled images; I think this is Jonas' critique}

% \todo[inline]{SE: reference to appendix?}


% \todo[inline]{SE: are these zero scores accounted in the scores?  \\Leixin: the compile error rate is calculated by error cases count divided by 404 [all cases] }



% \subsection{Challenging Features}

% \paragraph{More features worse performance?}

% \paragraph{Which feature is the most challenging one?}

% \paragraph{For a specific model, is there a specific challenging feature?}

% \todo[inline]{SE: the pair agreements are averaged?}




==> structure/table-example.tex <==
%\begin{table}[t!]
\begin{tabularx}{\textwidth}{|X|X|X|}
\hline
\textbf{Column 1} & \textbf{Column 2} & \textbf{Column 3} \\ \hline
This is a long text that adjusts to the column width. & Short text. & Another long text that adjusts dynamically. \\ \hline
More text. & Even more text. & Final column content. \\ \hline
\end{tabularx}
%\caption{Illustration of constructing generation queries.}
%\label{tab:prompt_template}
%\end{table}

==> structure/table-example_copy.tex <==
\begin{table}[t!]
\tiny
\centering
\begin{tabularx}{.9\textwidth}{>{\raggedright\arraybackslash}m{0.6in}>{\raggedright\arraybackslash}m{1.2in}>{\raggedright\arraybackslash}m{0.9in}>
{\raggedright\arraybackslash}m{1.4in}>{\raggedright\arraybackslash}m{1.2in}}
\hline
\\[0.1ex]
\textbf{Object Type} & \textbf{Query Template} & \textbf{Attribution} & \textbf{Generation Query} & \textbf{Understanding Dimension}\\[2ex]
\hline
\vspace{3px}2D shape &\vspace{3px} A/An \{object\} with a/an \{color\} border.
 &\vspace{3px} circle, blue &\vspace{3px} A circle with a blue border. & Attribute \\[1ex]
\hline
\vspace{3px}3D shape &\vspace{3px} Two \{color\} spaces divide a/an \{3D-object\} into four parts. \vspace{1px}&\vspace{3px} blue, pyramid & \vspace{3px}Two blue spaces divide a pyramid into four parts. & Attribute, Numeric \vspace{1px}\\[1ex]
\hline
\vspace{3px}Chart \vspace{3px}& \vspace{3px}In a bar chart, a/an \{color-1\} bar is to the right of a/an \{color-2\} bar, and the leftmost bar is the \{tallest/shortest\} in the chart.\vspace{3px} &\vspace{3px} blue, orange, tallest \vspace{3px} & \vspace{3px}In a bar chart, a blue bar is to the right of an orange bar, and the leftmost bar is the tallest in the chart. & Attribute, Numeric, Spatial \vspace{2px}\\[2.5ex]
\hline
\vspace{3px}Graph theory representation \vspace{1px}&\vspace{3px} A binary tree with a total of \{number\} nodes. & \vspace{3px}12 \vspace{1px}& \vspace{3px}A binary tree with a total of 12 nodes.& Numeric \vspace{1px} \\[2ex]
\hline
\vspace{3px}Matrix & \vspace{3px}A \{number\_1\}-by-\{number\_2\} matrix. &\vspace{3px} 6, 3 &\vspace{3px} A six-by-three matrix. &Numeric \\[1ex]
\hline
\vspace{3px}Real-life object &\vspace{3px} There are \{number-1\} boxes on a \{number-2\} degree slope. &\vspace{3px} 4, 30 & \vspace{3px}There are 4 boxes on a 30 degree slope.&Numeric, Spatial \\[1ex]
\hline
\vspace{3px}Table \vspace{1px}& \vspace{3px}A table with \{number-1\} rows and \{number-2\} columns. The row index is marked in the first column. \vspace{1px}& \vspace{3px}3, 5 \vspace{1px}&\vspace{3px} A table with three rows and five columns. The row index is marked in the first column.&Attribute, Numeric, Spatial\vspace{1px} \\[1.5ex]
\hline
\vspace{3px}Annotation & \vspace{3px}The English text (the name of the object) is \{preposition\} the \{object\}. & \vspace{3px}to the left of, triangle & \vspace{3px}The English text (the name of the object) is to the left of the triangle. & Spatial\\[1ex]
\hline 
\vspace{3px}Function \& Coordinate &\vspace{3px} y = \{function\} and its inverse function. & \vspace{3px}3\textasciicircum{x} &\vspace{3px} y = 3\textasciicircum{x} and its inverse function. & Numeric
\\[1ex]
\hline\\[0.01ex]
\end{tabularx}
\caption{Illustration of constructing generation queries.}
\label{tab:prompt_template}
\end{table}
